Multi-FedLS: a Framework for Cross-Silo Federated Learning Applications on Multi-Cloud Environments

Federated Learning (FL) is a distributed Machine Learning (ML) technique that can benefit from cloud environments while preserving data privacy. We propose Multi-FedLS, a framework that manages multi-cloud resources, reducing execution time and financial costs of Cross-Silo Federated Learning applications by using preemptible VMs, cheaper than on-demand ones but that can be revoked at any time. Our framework encloses four modules: Pre-Scheduling, Initial Mapping, Fault Tolerance, and Dynamic Scheduler. This paper extends our previous work \cite{brum2022sbac} by formally describing the Multi-FedLS resource manager framework and its modules. Experiments were conducted with three Cross-Silo FL applications on CloudLab and a proof-of-concept confirms that Multi-FedLS can be executed on a multi-cloud composed by AWS and GCP, two commercial cloud providers. Results show that the problem of executing Cross-Silo FL applications in multi-cloud environments with preemptible VMs can be efficiently resolved using a mathematical formulation, fault tolerance techniques, and a simple heuristic to choose a new VM in case of revocation.

==> old_articles/draft.tex <==
% % Complement SBAC and WCC in the end and rearrange these paragraphs
% The literature shows works focusing on scheduling and resource management of FL jobs~\cite{yang2020scheduling, xia2020multi_armed_scheduling, ren2021joint_resource_allocation, buyukates2021timely_communication, pilla2021optimal} on Cross-Device Federated Learning scenarios. In this scenario,  such resources, hundreds or thousands of connected devices, are low-powered that frequently become offline during the training process.
% % commentaries of these references above

% % Restructure next paragraphs
% Regarding distributed machine learning, various works focus on the job scheduling problem of multiple ML jobs allocated among a limited number of resources~\cite{zhang2020online_heterogeneous_distributed, liu2020distributed_ml_networks, yu2021distributed_ml_locality}. Few of them handle the scheduling problem on unique distributed ML applications.

% The scheduling and resource provisioning problems of distributed Machine Learning (ML) applications~\cite{mohamadi2019distributed_ml_stragglers, liu2020distributed_ml_networks, yu2021distributed_ml_locality} 
% can be related to the scheduling in Cross-Silo FL applications if we assume the clients' jobs are always available.

% The showed solution by
% Amiri~\etal~\cite{mohamadi2019distributed_ml_stragglers} accepts tasks (workers) presenting sporadic slowness due to temporary network disconnection. The central dataset is divided into small $n$ chunks to overcome such problems. 

% Each worker should compute them sequentially. The server task sends chunks to multiple workers and waits for $k$ results, $k \leq n$. To reduce the average completion time, the authors propose two scheduling schemes to assign chunks for workers. The data-sharing approach does not work for Federated Learning scenarios because data privacy and heterogeneity are essential concerns. 

% To the best of our knowledge, few works in the literature focus on Cross-Silo Federated Learning \cite{rajendran2021cloud, huang2021personalized_cross_silo, li2021federated}.
% % commentaries of references above

\chapter{Related work}
\label{chap:related_work}

Since the first FL algorithm, FedAvg, proposed by McMahan~\etal~\cite{mcmahan2017communication}, several works present optimizations and new aggregation strategies to the FL execution scheme~\cite{li2018federated, shaoxing2019learning_attentive, jinijn2020ternary_compression, chen2020layerwise}. However, these optimizations consider a Cross-Device FL setting. There are usually hundreds or thousands of clients that can turn off during the FL execution. For example, Li~\etal~\cite{li2018federated} present FedProx, an optimized version of FedAvg that avoids the delay presented by slower devices by allowing them to train a fraction of the local epochs within a communication round, and Chen~\etal~\cite{chen2020layerwise} propose an asynchronous learning strategy to reduce the communication cost of the FL execution when using a DNN model. 

In this paper, we focus on the Cross-Silo FL architecture, which is characterized by fewer but more powerful clients, with machines or even clusters to execute the training with a stable network connection. Therefore, the server assumes that all clients will always be available, and it does not need to use any optimizations regarding the number of clients or their eventual disconnection within a communication round. Besides, we present a resource manager that can handle any Cross-Silo FL application and, thus, we do not take advantage of any server aggregation scheme that focuses on a specific ML model.

Regarding the main scheduling perspectives related to FL, there are two: one considers Cross-Device FL while the other deals with Cross-Silo FL. In the related literature, most papers treat Cross-Device FL, whereas we focus on the Cross-Silo FL architecture, as explained before. The scheduling perspective in a Cross-Device FL scheme is related to the selection of a client fraction in each communication round~\cite{yang2020scheduling, xia2020multi_armed_scheduling, ren2021joint_resource_allocation, buyukates2021timely_communication, pilla2021optimal}, due to the characteristics of the Cross-Device clients. Low-powered resources, like mobile phones or IoT devices, usually connect to other devices or the Internet through an unstable wireless network, frequently becoming offline in the middle of the training process. 

Yang~\etal~\cite{yang2020scheduling} propose an FL algorithm that divides the global model into smaller parts trained uniquely by each device's local dataset. They demonstrate that the aggregation of these smaller parts leads to a higher convergence rate. Besides, Yang~\etal~analyse the convergence rate of their algorithm using three different scheduling policies for sampling clients: random scheduling, round-robin, and proportional fair. 
%The random scheduling chooses $k$ clients per communication round from all clients,  while the round-robin policy divides all clients into $G$ groups and chooses one group per communication round. The proportional fair policy considers the response time of each client to select the $k$ participating ones.
Xia~\etal~\cite{xia2020multi_armed_scheduling} present a Multi-Armed Based client scheduling policy. The Multi-Armed Based problem is composed of sequential decision problems. In each of them, the algorithm needs to decide from a finite pool of resources which one to use, considering the results of the previous time steps~\cite{lai1985multi_armed_based_problem, bubeck2012regret}. The authors in~\cite{xia2020multi_armed_scheduling} do not assume any knowledge of the wireless channels state and focus on minimizing the total wall-clock time consumption within a given number of communication rounds. % They present scheduling policies for two different scenarios of data distribution: the ideal one, when all clients have homogeneous and equal class distribution among them, and the non-IID one, the one more realistic.
Ren~\etal~\cite{ren2021joint_resource_allocation} formulate a mixed-integer non-linear problem in an FL scenario where the IoT devices send their raw data to edge servers that train it locally. The proposed problem minimizes system and learning costs by optimizing computation frequency, bandwidth and subcarrier assignment, and transmission power allocation. % They simplify this original problem using decomposition and firstly reach a closed-form solution for the bandwidth assignment problem. Then, the authors use an iterative algorithm to solve the other optimization issues.
Buyukates and Ulukus~\cite{buyukates2021timely_communication} focus on applications that use temporal data to predict something. For example, an application that uses the location and speed of users to avoid traffic jams when giving directions. In this application, the data recently produced has a bigger impact than the older ones. Thus, the authors select $m$ clients to participate in each communication round and make the server aggregate only the $k$ clients ($k < m$) with the earliest data. % They also formulate the optimal $m$ and $k$ values given the total number of clients $n$ and present numerical results for $n = 100$.

In this work, we focus on scheduling Cross-Silo FL applications in clouds. In a Cross-Silo scenario, the clients are institutions, and they usually have more computational power and stabler network connection than Cross-Device clients. Thus, we assume that clients are available at all times and they all participate in each communication round and our scheduling problem consists of finding the optimal placement of each participating client and the server, aiming at minimizing the execution and financial costs. 

With the assumption that the clients are always available, the scheduling of Cross-Silo FL applications is related to scheduling distributed ML applications. The majority of works in the literature focuses on determining the optimal number of parameter servers and workers per job when scheduling multiple ML jobs in limited resources~\cite{zhang2017slaq, bao2018online_scheduling_distributed, zhang2020online_heterogeneous_distributed}. They assume that all workers will have the same amount of data and allocate them as close as possible. These two assumptions are the main difference from our work, where each client stores their heterogeneous private datasets in different cloud regions or even cloud providers. However, some recent papers consider stragglers~\cite{mohamadi2019distributed_ml_stragglers}, the network performance~\cite{liu2020distributed_ml_networks}, or locality awareness~\cite{yu2021distributed_ml_locality} being closer to ours.

Amiri~\etal~\cite{mohamadi2019distributed_ml_stragglers} consider transient stragglers among workers during the distributed ML training. Transient stragglers are workers with sporadic slowness due to temporary network disconnection. To handle them, the authors divide the central dataset into $n$ small chunks assuming that each worker will compute over a number of them sequentially. Then, the parameter server sends each piece to multiple workers and waits for $k$ results from different chunks, $k \leq n$. One important aspect of this work is the data exchange between the tasks, prohibitive in a Federated Learning scenario. Thus, the whole FL execution needs to consider the stragglers' execution time.

Liu~\etal~\cite{liu2020distributed_ml_networks} focus on the impact of Optical Circuit Switches (OCSes) on multiple distributed ML training jobs execution in a data center or cluster. OCSes are energy-saving and high-performance switches that use light properties to make light passively flow in the desired direction. Hence, each port of an OCS switch only supports communication to another port in a single way. If the application needs to send any message in another direction to another port, the OCS switch needs time to reconfigure itself. Thus, Liu~\etal~proposed two scheduling policies that consider the reconfiguration time. Besides handling possible network contention, the authors assume that all workers will have the same dataset size, class distribution, and computational power, which is not always valid in a Federated Learning scenario due to privacy concerns.

Yu~\etal~\cite{yu2021distributed_ml_locality} formulate an optimization model to allocate tasks from different distributed ML jobs into a set of physical machines regarding resource and locality-aware constraints. Their model needs to know when each ML training job arrives and determines the best allocation scheme for all workers and parameter servers for each ML training job minimizing the communication time between them. They assume that the parameter server and the workers can co-locate in the same physical machine. They also consider that communication happens after training a few samples instead only at the end of a whole epoch. Despite presenting a locality-aware scheduling problem, this work has assumptions that cannot be valid in a Federated Learning scenario. First, they assume a central dataset, which is impossible in FL. Second, Yu~\etal~assume that the communication between workers and parameter server happens more frequently than in a FL scenario, where clients and the server communicate only after a few training epochs. Finally, the co-location of clients and servers in Federated Learning can help malicious clients discover other clients' information using reverse engineering on the weights updates~\cite{truong2021privacy_preservation_fl}. Thus, it is safer to allocate tasks to different resources in FL.


\section{Scheduling Distributed Machine Learning Jobs} \label{sec:related_work_scheduling_distributed_ml}

The majority of works focus on determining the optimal number of parameter servers and workers per job when scheduling multiple ML jobs in limited resources~\cite{zhang2017slaq, bao2018online_scheduling_distributed, zhang2020online_heterogeneous_distributed}. They assume that all workers will have the same amount of data and allocate them as close as possible. These two assumptions are the main difference from our work, where each client stores their heterogeneous private datasets in different cloud regions or even cloud providers. However, some recent papers consider stragglers~\cite{mohamadi2019distributed_ml_stragglers}, the network performance~\cite{liu2020distributed_ml_networks}, or locality awareness~\cite{yu2021distributed_ml_locality} being closer to ours.

Amiri~\etal~\cite{mohamadi2019distributed_ml_stragglers} consider transient stragglers among workers during the distributed ML training. Transient stragglers are workers with sporadic slowness due to temporary network disconnection, as an example. To handle them, the authors divide the central dataset into $n$ small chunks assuming that each worker will compute over a number of them sequentially. Then, the parameter server sends each piece to multiple workers and waits for $k$ results from different chunks, $k \leq n$. The authors present the proposed system model and theoretical analysis for the minimum average completion time. Finally, they explain two scheduling schemes for chunks assignment to the workers, and their experimental results present better completion time than other algorithms in the literature. One aspect of this work is the data exchange between the tasks, prohibitive in a Federated Learning scenario. Thus, the whole FL execution needs to consider stragglers' execution time.

Liu~\etal~\cite{liu2020distributed_ml_networks} focus on the impact of Optical Circuit Switches (OCSes) on multiple distributed ML training jobs execution in a data center or cluster. OCSes are energy-saving and high-performance switches that use light properties to make light passively flow in the desired direction. Hence, each port of an OCS switch only supports the communication to another port in a single way. If the application needs to send any message in another direction to another port, the OCS switch needs time to reconfigure itself. Thus, Liu~\etal~proposed two scheduling policies that consider the reconfiguration time. The Heaviest-Load-First (HLF) policy to schedule tasks within the same distributed ML job, and Shortest Weighted Remaining Time First (SWRT) to schedule different training interleaving their computation and communication phases. Besides handling possible network contention, the authors assume that all workers will have the same dataset size, class distribution and computational power, which is not always valid in a Federated Learning scenario due to privacy concerns.

Yu~\etal~\cite{yu2021distributed_ml_locality} formulate an optimization model to allocate tasks from different distributed ML jobs into a set of physical machines regarding resource and locality-aware constraints, named the offline distributed Machine Learning resource scheduling problem (DMLRS). DMLRS needs to know when each ML training job arrives and determines the best allocation scheme to all workers and parameter servers to each ML training job minimizing the communication time between them. They assume that the parameter server and the workers can co-locate in the same physical machine. They also consider that communication happens after training a few samples instead only at the end of a whole epoch. Besides, the authors propose an online scheduling algorithm based on a reformulation of DMLRS to a primal-dual and online problem. Despite presenting a locality-aware scheduling problem, this work has assumptions that cannot be valid in a Federated Learning scenario. First, they assume a central dataset, which is impossible in FL. Second, Yu~\etal~assume that the communication between workers and parameter server happens more frequently than in a FL scenario, where clients and the server communicate only after a few training epochs. Finally, the co-location of clients and servers in Federated Learning can help malicious clients discover other clients' information using reverse engineering on the weights updates~\cite{truong2021privacy_preservation_fl}. Thus, it is safer to allocate tasks to different resources in FL.

\section{Distributed Machine Learning and Federated Learning on Clouds} \label{sec:related_work_fl_ml_clouds}

Regarding the papers handling distributed Machine Learning on Clouds, most of them use cloud services as a tool to evaluate their scheduling proposal~\cite{mohamadi2019distributed_ml_stragglers, yu2021distributed_ml_locality} or to verify the central dataset integrity~\cite{zhao2020distributed_ml_integrity_verification}. We found few research papers that consider aspects of Cloud Computing to propose their solution~\cite{zhang2020machine_learning_volatile, duong_quang2018distributed_ml_iaas, duong2019fc2, wagenlander_2020_spotnik}. However, the authors assume the equal division of the central dataset among workers, and they usually use a single region to allocate all cloud resources. These facts reinforce that distributed ML do not concern about data privacy and heterogeneity, which are the essence of Federated Learning.

Zhang~\etal~\cite{zhang2020machine_learning_volatile} consider Spot (or preemptible) cloud instances to train distributed ML tasks. Cloud providers offer their spare capacity as preemptible instances with a huge discount, but they can revoke them at any time. As there is no guarantee that all workers from a distributed ML job will be available throughout the execution, Zhang~\etal study the convergence of classical algorithms to distributed ML training when the number of workers varies. They present a formula to obtain the optimal number of workers to deploy so that the algorithm does not diverge. They also validate their results using Amazon EC2~\cite{aws_ec2} Spot instances.

Duong and Quang~\cite{duong_quang2018distributed_ml_iaas, duong2019fc2} present a system to execute distributed ML jobs into on-demand instances of a cloud provider called  FC$^2$. They implement a simple web interface so that ML practitioners add their ML model characteristics and available budget, and FC$^2$ calculates the total number of workers to deploy into different instance types from a pool of available ones. The authors also implement two heuristics to recommend the instances, one considering the execution time per instance and the other the instances' bandwidth. Doung and Quang execute all results using Amazon EC2~\cite{aws_ec2} instances.

Wagenländer~\etal~\cite{wagenlander_2020_spotnik} propose Spotnik to deal with instance revocations due to preemptible cloud instances in distributed ML training. They assume a decentralized training approach in which the workers communicate with each other in a pre-defined ring pattern to aggregate their results. Thus, in the communication phase, if a worker $w_i$ cannot reach its neighbor $w_j$, it assumes a revocation occurred, ignores the changes in the current iteration, removes $w_j$ from the known topology, and propagates this change. Spotnik also adapts its training method accordingly to the current number of workers. If the number of workers is low, Spotnik uses synchronous strategies to calculate the aggregated results and, if the number of workers is high, Spotnik uses asynchronous ones.

To the best of our knowledge, few works tackle the problem of federated learning on clouds in the related literature. 

Liu~\etal~\cite{liu2020client} present a hierarchical FL architecture with mobile devices as clients. Their principle idea is the addition of an edge layer of servers. These edge servers aggregate the results of a fraction of the clients and send their aggregation to a central cloud server. Then, this central server aggregates the results of all edge servers and, consequently, all clients. The authors present the algorithm to this architecture and its convergence analysis in the paper. However, they only show simulation results to prove their convergence analysis.

Fang~\etal~\cite{FANG2020101889} propose an architecture for Federated Learning in the cloud focusing on privacy. Their architecture consists of a central server on the cloud with clients that uses ElGamal encryption~\cite{crypt_elgaman} to encrypt all messages. They present how the server and clients exchange their encryption keys and how the framework works. The authors compare their solution theoretically with other privacy-concerning deep learning methods. Besides, they simulate the FL environment in a local machine and present the accuracy, execution times, and messages size of each one.

The only found work that runs a FL approach in a cloud environment is the work of Rajendran~\etal~\cite{rajendran2021cloud}. They presented the results of both implemented models in a scenario with two clients in a simulated environment and on the Microsoft Azure Cloud Databricks~\cite{azure_databricks}, an open-source tool for data engineering and collaborative data science, to exchange the ML model between two institutions.

In this work, we focus on synchronous FL training on VMs in the cloud and how we can schedule each actor (the server and clients) to minimize the total execution costs respecting the location of each client's dataset. 


\section{Summary}


As presented in this chapter, most work on Federated Learning in the literature tackles the clients' unstable network from the Cross-Device architecture. In this scenario, the server needs to sample a fraction of clients in each communication round, as there are usually hundreds or thousands of devices connected. We focus on Cross-Silo FL, which assumes fewer clients and a better network connection in the present work. The clients are dedicated machines or clusters, and the server usually samples all to participate in each round as they are available throughout the entire execution. Moreover, we intend to create a generic Cross-Silo FL scheduler and, thus, we cannot take advantage of algorithms that focus on CNNs or RNNs. 

Thus, Table \ref{tab:papers_fl} presents all previously described works regarding Federated Learning compared to ours. We describe the ML algorithm that each work implements (ML model), whether the authors evaluated their proposal using simulation or real-world schemes (Environment), and the FL type the paper focus. For the papers proposing scheduling solutions, we also present the minimization objective and the criteria used in their solution. If the authors do not mention which ML model they focus on, we use the N/S value.

Regarding the presented works on scheduling distributed Machine Learning (DML) jobs, they focus on three aspects that our scheduler could consider: non-persistent stragglers~\cite{mohamadi2019distributed_ml_stragglers}, network performance~\cite{liu2020distributed_ml_networks}, and locality of the dataset and tasks~\cite{yu2021distributed_ml_locality}. Table \ref{tab:papers_distributed_ml} compares these works presenting their main characteristics. We present the minimization objective of each paper, how the authors solved their optimization problem (Solution), in which environment they tested the solution, and if the authors considered an online or offline problem. An online optimization problem is when new tasks can arrive during the execution, and, in the offline approach, all tasks' information is already available before the scheduling.

==> old_articles/dynamic_scheduler_old.tex <==
\subsection{Fault Tolerance module}
(Rafaela: Missing client checkpoint)

% Thesis Proposal text
To reduce costs, Multi-FedLS uses preemptible (or spot) VMs. Cloud providers offer these VMs at a discount compared to on-demand VMs. However, the preemptible VMs can be revoked at any time by the cloud provider and, thus, our application needs to handle possible revocation events. AWS usually sends a two-minute notification to the selected VM to notify us about the revocation, but Google Cloud gives us only 30 seconds to terminate the VM. Thus, we need to prepare our application for possible faults during the execution. The failure of a client or the server in an FL application impacts differently on the FL execution. 
% WCC text modified
When Flower detects a client failure during a single communication round, the server ignores the faulty client by aggregating only the results from the other ones and waits for the defined minimum number of available clients to start a new communication round. In cross-silo FL, our aimed type of FL, there are usually few clients, and losing one of them can compromise the learning outcomes. So, the FL server always waits for all clients to be available to start the next communication round. 

While Flower handles a client's error smoothly, there is no fault tolerance implemented when the server fails and all clients stop their execution after receiving an error. Thus, Multi-FedLS needs to handle possible server revocations by implementing fault-tolerant techniques on the server side. Although Flower does not have an automatic way to save the model updates on the server side after each communication round, it allows the users to modify the server code to implement the model checkpoint during the server's aggregation phase\footnote{https://flower.dev/docs/saving-progress.html}. In our framework, we take advantage of this feature asking for the server to checkpoint every $X$ rounds and whenever there is a new stored checkpoint on the server VM's disk, we transfer it to another location, which is a storage service, or an extra VM.

During the FL execution, the Fault Tolerance module monitors all tasks and handles eventual VMs revocations and runtime errors. When the FT module detects any revocation or error, it triggers the Dynamic Scheduler module to select a new VM for the affected task. The details of our Dynamic Scheduler module are described in the next subsection. When all tasks finish the FL execution, our Fault Tolerance module stops the monitoring and starts the VMs termination process.

% Rafaela: Talk about client checkpoint process

\subsection{Dynamic Scheduler module}
(Rafaela: Draft)

When the Fault Tolerance module calls the Dynamic Scheduler, it informs the affected task type. Depending on this type, the Dynamic Scheduler uses different greedy algorithms to choose the new instance to restart the affected task. It also takes advantage of the metrics computed by the Pre-Scheduling and the Initial Mapping modules and adapts the mathematical formulation. 
% Rascunho
Both algorithms compute the new expected makespan and expected costs in a single FL round using an instance $vm_{jkl}$ to the affected task $t$ and, to make the greedy algorithms more understandable, we present these computations separately. Thus, Algorithm \ref{alg:new-makespan} computes the new makespan using $t$ as the affected task (which can be $s$ for the server or $c_i$ for client $i$) and $vm_{jkl}$ as the instance to be allocated to task $t$. 

\begin{algorithm}
 \caption{Function computing new makespan using $vm_{jkl}$ in task $t$} \label{alg:new-makespan}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE $t, vm_{jkl}$
\STATE $max\_makespan \gets -\infty$
\IF{$t = s$ }\COMMENT{Affected task is the server} \label{alg:new-makespan-task-type}
    \FOR{$c_i \in C$} \label{alg:new-makespan-loop-server-init}
        \STATE $current\_vm_{mno} \gets current\_map_{c_i}$
        \STATE $total\_time \gets t\_exec_{imno} + t\_comm_{mnjk} + t\_aggreg_{jkl}$
        \IF{$total\_time > max\_makespan$}
            \STATE $max\_makespan \gets total\_time$
        \ENDIF
    \ENDFOR \label{alg:new-makespan-loop-server-end}
\ELSE{ }\COMMENT{Affected task is client $c_t$} \label{alg:new-makespan-client}
    \STATE $current\_server\_vm_{mno} \gets current\_map_{s}$
    \STATE $max\_makespan \gets t\_exec_{tjkl} + t\_comm_{jkmn} + t\_aggreg_{mno}$
    \FOR{$c_i \in C\backslash \{c_t\}$} \label{alg:new-makespan-loop-client-init}
        \STATE $current\_vm_{pqr} \gets current\_map_{c_i}$
        \STATE $total\_time \gets t\_exec_{ipqr} + t\_comm_{pqmn} + t\_aggreg_{mno}$
        \IF{$total\_time > max\_makespan$}
            \STATE $max\_makespan \gets total\_time$
        \ENDIF
    \ENDFOR \label{alg:new-makespan-loop-client-end}
\ENDIF
\STATE \textbf{return} $max\_makespan$
\end{algorithmic}
\end{algorithm}

As explained in Section \ref{sec:initial-mapping}, the makespan of an FL round is determined by the client which takes longer to send its weights to the server. A client delay can be related to two different things: a longer training time or a longer communication time. Thus, in our algorithm, we compute the makespan by obtaining the bigger total time a single client needs to train and communicate with the server along with the server's aggregation time. However, as we are changing the instance of a specific task, we need to reflect the makespan to compute this task's new execution time. So, first, we check if the affected task is the server (Line \ref{alg:new-makespan-task-type}) or a client (Line \ref{alg:new-makespan-client}). If the affected task is the server, then $vm_{jkl}$ is the new server instance and we execute the loop in Lines \ref{alg:new-makespan-loop-server-init}-\ref{alg:new-makespan-loop-server-end} to compute the total expected execution time of each client and stores the highest one as the new makespan. Otherwise, if the affected task is a client, we first get the current server instance in variable $current\_server\_vm_{mno}$ and compute the makespan of the current affected task using $vm_{jkl}$ as the client's instance. Then, we execute the loop in lines \ref{alg:new-makespan-loop-client-init}-\ref{alg:new-makespan-loop-client-end} to check if any of the current clients has a higher makespan. 

Next, we present the algorithm to calculate the new cost in Algorithm \ref{alg:new-cost}, which receives the same inputs as the previous algorithm, $t$ and $vm_{jkl}$, and also the makespan in $makespan$.

\begin{algorithm}
 \caption{Function computing new expected cost using $vm_{jkl}$ in task $t$ and expected makespan in $makespan$} \label{alg:new-cost}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE $t, vm_{jkl}, makespan$
\STATE $total\_cost \gets 0.0$
\IF{$t = s$ }\COMMENT{Affected task is the server}
    \STATE $total\_cost \gets total\_cost + cost_{jkl} \times makespan$
    \FOR{$c_i \in C$}
        \STATE $current\_vm_{mno} \gets current\_map_{c_i}$
        \STATE $total\_cost \gets total\_cost + cost_{mno} \times makespan$
        \STATE $total\_cost \gets total\_cost + comm_{jm}$ \COMMENT{$comm_{jm}$ as Equation \ref{}}
    \ENDFOR
\ELSE{ }\COMMENT{Affected task is client $c_t$}
    \STATE $current\_server\_vm_{mno} \gets current\_map_{s}$ \label{alg:new-cost-server-client}
    \STATE $total\_cost \gets total\_cost + cost_{jkl} \times makespan$
    \STATE $total\_cost \gets total\_cost + comm_{mj}$ \COMMENT{$comm_{mi}$ as Equation \ref{}}
    \FOR{$c_i \in C\backslash \{c_t\}$}
        \STATE $current\_vm_{pqr} \gets current\_map_{c_i}$
        \STATE $total\_cost \gets total\_cost + cost_{pqr} \times makespan$
        \STATE $total\_cost \gets total\_cost + comm_{mp}$ \COMMENT{$comm_{mp}$ as Equation \ref{}}
    \ENDFOR
\ENDIF
\STATE \textbf{return} $total\_cost$
\end{algorithmic}
\end{algorithm}

The total cost in a single FL round comprises the execution cost of each task and the message exchange costs of each client to the server. Thus, in Algorithm \ref{alg:new-cost} we first compute the execution cost of the server and then we compute the execution and message exchange costs of each client. The execution cost of an instance is the multiplication of the makespan and the instance cost and the message exchange cost is computed using Equation \ref{}, the cost to exchange the FL messages between the server provider and the client one. Equally to the previous algorithm, when the affected task $t$ is the server we already have the server provider $p_j$ from the input instance $vm_{jkl}$. Otherwise, if the affected task is a client, we get the current server instance in Line \ref{alg:new-cost-server-client} to use its provider $p_{m}$ as the server's provider.

Now we present the greedy heuristic for choosing a new server or a new client when after a fault. If the affected task is the server $s$, we execute Algorithm \ref{alg:new-server} to choose the new server instance. Otherwise, if the 

\begin{algorithm}
 \caption{Greedy heuristic for choosing a new server} \label{alg:new-server}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE $I_{s}, old\_vm_{jkl}$
\STATE $remove\_vm\_from\_set(I_{s}, old\_vm_{jkl})$
\STATE $min\_value \gets \infty$
\FOR{\textbf{each} $vm_{mno} \in I_{s}$}
    \STATE $makespan \gets computes\_new\_makespan(s, vm_{mno})$ \COMMENT{Algorithm \ref{alg:new-makespan}}
    \STATE $cost \gets compute\_expected\_cost(makespan, s, vm_{mno})$ \COMMENT{Algorithm \ref{alg:new-cost}}
    \STATE $value \gets \alpha \times (cost / max\_cost) +  (1 - \alpha) \times (makespan / max\_makespan)$
    \IF {$value < min\_value$}
        \STATE $new\_instance \gets vm_{mno}$
        \STATE $min\_value \gets value$
    \ENDIF
\ENDFOR
\STATE \textbf{return} $new\_instance$
\end{algorithmic}
\end{algorithm}

% If the task is a client, the greedy heuristic chooses the VM that results in the lower expected execution time and communication time to the actual server location. Algorithm \ref{alg:new-client} presents the details of the greedy heuristic to choose a new VM for client $c_i$, which receives as input $I_{c_i}$ being the current set of VMs for client $c_i$, $old\_vm_{jkl}$ being the current revoked VM, and $prov_{s}$ and $reg_{s}$ being the current provider and region for the server.


\begin{algorithm}
\caption{Greedy heuristic for choosing a new client} \label{alg:new-client}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE $c_i, I_{c_i}, old\_vm_{jkl}$
\STATE $remove\_vm\_from\_set(I_{c_i}, old\_vm_{jkl})$
\STATE $min\_value \gets \infty$
\FOR{\textbf{each} $vm_{mno} \in I_{c_i}$}
    \STATE $makespan \gets computes\_new\_makespan(c_i, vm_{mno})$ \COMMENT{Algorithm \ref{alg:new-makespan}}
    \STATE $cost \gets compute\_expected\_cost(makespan, c_i, vm_{mno})$ \COMMENT{Algorithm \ref{alg:new-cost}}
    \STATE $value \gets \alpha \times (cost / max\_cost) +  (1 - \alpha) \times (makespan / max\_makespan)$
    \IF {$value < min\_value$}
        \STATE $new\_instance \gets vm_{mno}$
        \STATE $min\_value \gets value$
    \ENDIF
\ENDFOR
\STATE \textbf{return} $new\_instance$
\end{algorithmic}
\end{algorithm}

% The first step in Algorithm \ref{alg:new-client} is to remove the revoked VM from the set of possible VMs the client $c_i$ can execute. From previous experiments, we observed that once the instance type is revoked in a region, it cannot be reallocated in the same region~\cite{brum2021fault}. Thus, we assume this behavior to all cloud providers and remove the $old\_vm_{jkl}$ from $I_{c_i}$. Note that we do not use the same set for all clients as they can have different dataset sizes which correspond to different expected execution times. After removing the revoked VM, our algorithm starts the loop iterating on all VMs from $I_{c_i}$ (lines 3-9 of Algorithm \ref{alg:new-client}) to select the fastest VM in the set. The communication round of an FL application is always bounded by the client that takes longer to send the message to the server, and that is the reason we add the communication time between the compared VM and the server to the total expected execution time. If the fastest VM of the set is too far from the server, its communication time can take longer than a slightly slower VM that is closer to the server.

% (Rafaela: Missing description of greedy heuristic to choose a new server)

==> old_articles/related_work_proposal.tex <==
\chapter{Related work}
\label{chap:related_work}

There are two main scheduling perspectives related to Federated Learning (FL): one considers Cross-Device FL while the other deals with Cross-Silo FL. In the related literature, most papers treat Cross-Device FL. The main challenge on the Cross-Device FL architecture is handling low-powered devices that can disconnect at any time due to unstable network connections. Thus, most recent papers focus on either the proposal of new algorithms to the server aggregation or the scheduling of clients to be sampled in a Cross-Device FL application. Section \ref{sec:related_work_federated_learning} describes the new algorithms, while Section \ref{sec:related_work_scheduling_fl} presents the scheduling papers on Cross-Device FL.

Our work focuses on Cross-Silo FL architectures, where the clients are institutions. The scheduling problem of Cross-Silo FL applications consists of finding the optimal placement of each participating client, aiming at minimizing the execution and financial costs. Section \ref{sec:related_work_cross_silo_fl} presents current work focused on Cross-Silo FL applications. The scheduling of Cross-Silo FL applications can be related to scheduling distributed Machine Learning (ML) applications as there is the assumption that workers are always available. Thus, Section \ref{sec:related_work_scheduling_distributed_ml} presents recent work on scheduling distributed ML applications. Finally, Section \ref{sec:related_work_fl_ml_clouds} introduces papers that consider distributed ML and FL executed on cloud environments.

\section{Algorithms of Federated Learning scenario} \label{sec:related_work_federated_learning}

We describe in this section works that propose new algorithms to Cross-Device FL. These algorithms focus on server aggregation when low-powered clients disconnect at any time during the FL training.

Since the first FL algorithm, FedAvg, presented by McMahan~\etal~\cite{mcmahan2017communication}, several works present optimizations and new aggregation strategies~\cite{li2018federated, shaoxing2019learning_attentive, jinijn2020ternary_compression, chen2020layerwise}. However, these optimizations consider a Cross-Device FL setting. There are usually hundreds or thousands of clients, and they can turn off during the FL execution.

Li~\etal~\cite{li2018federated} show FedProx, an optimized version of FedAvg that avoids the delay presented by slower devices. FedProx allows the devices to train a fraction of the local epochs within a communication round. The authors also deal with the global model divergence when the local epoch number in each round is high. They add a proximal term into the training function focusing on reducing the training updates. The authors present a better training loss than the FedAvg algorithm, but they claim that the fraction of local epochs accepted and the proximal term need tuning for each new FL model. Besides, they simulated all their experiments in a single machine.

Ji~\etal~\cite{shaoxing2019learning_attentive} present an optimization to the server aggregation of Federated Learning focused on the problem of Natural Language Processing. The models used in this area are the Recurrent Neural Networks (RNNs), a type of DNNs. Their principal characteristic is that they can save information about a sample to influence the result of the next ones. 
The authors use an attentive mechanism to highlight the main model layers with weights updated more frequently. They conducted the experiments in a single machine and presented only the perplexity metric used to compare natural language models.

Xu~\etal~\cite{jinijn2020ternary_compression} consider a ternary compression in the model weights to reduce the communication costs among the server and clients. They accomplish the theoretical analysis of their algorithm and experiment on a hybrid environment. Their experiments used publicly available datasets trained in two Convolutional Neural Networks (CNNs), a type of DNNs specialized in extracting features of images. The authors present their experiments in four machines with ten clients. They compare their algorithm to the FedAvg observing accuracy and communication costs. However, the authors did not make available their source code.

Chen~\etal~\cite{chen2020layerwise} propose an asynchronous learning strategy to reduce the communication cost of the FL execution. They categorize DNN layers into shallow and deep ones and use this categorization to update each layer category in a different frequency. The shallow layers are responsible for extracting general features found in different datasets and tasks, while deep layers focus on features specific to the current task. Thus, Chen~\etal~update the weights of the shallow layers in every communication round and update the deep layers only in the last communication rounds. They present evaluation results with 15 rounds, updating the deep layers in the final three, five, and seven. Besides, the authors describe a weighted aggregation strategy based on the last update time of each DNN layer. The FL server saves the last update round of each layer and aggregates the information of previous models into the current aggregation.

As our work focuses on Cross-Silo Federated Learning, the server can assume that all clients will always be available. Besides, we focus on scheduling general Cross-Silo FL applications and, thus, we cannot take advantage of the specificities of a CNN or an RNN. 

\section{Scheduling Cross-Device Federated Learning} \label{sec:related_work_scheduling_fl}

Although there is a vast literature in scheduling FL jobs~\cite{yang2020scheduling, xia2020multi_armed_scheduling, ren2021joint_resource_allocation, buyukates2021timely_communication}, most of them focus on the Cross-Device Federated Learning scenario. Low-powered resources, like mobile phones or IoT devices, usually connect to other devices or the Internet through an unstable wireless network, frequently becoming offline in the middle of the training process. Researchers use different scheduling policies to sample the clients in each communication round to tackle this problem.

Yang~\etal~\cite{yang2020scheduling} propose an FL algorithm that divides the global model into smaller parts trained uniquely by each device's local dataset. They demonstrate that the aggregation of these smaller parts leads to a higher convergence rate. Besides, Yang~\etal~analyse the convergence rate of their algorithm using three different scheduling policies for sampling clients: random scheduling, round-robin, and proportional fair. The random scheduling chooses $k$ clients per communication round from all clients,  while the round-robin policy divides all clients into $G$ groups and chooses one group per communication round. The proportional fair policy considers the response time of each client to select the $k$ participating ones.

Xia~\etal~\cite{xia2020multi_armed_scheduling} present a Multi-Armed Based client scheduling policy. The Multi-Armed Based problem is composed of sequential decision problems. In each of them, the algorithm needs to decide from a finite pool of resources which one to use, considering the results of the previous time steps~\cite{lai1985multi_armed_based_problem, bubeck2012regret}. The authors in~\cite{xia2020multi_armed_scheduling} do not assume any knowledge of the wireless channels state and focus on minimizing the total wall-clock time consumption within a given number of communication rounds. They present scheduling policies for two different scenarios of data distribution: the ideal one, when all clients have homogeneous and equally class distribution among them, and the non-IID one, the one more realistic.

Ren~\etal~\cite{ren2021joint_resource_allocation} formulate a mixed-integer non-linear problem in a FL scenario where the IoT devices send their raw data to edge servers train them locally. The proposed problem minimizes system and learning costs by optimizing computation frequency, bandwidth and subcarrier assignment, and transmission power allocation. They simplify this original problem using decomposition and firstly reach a closed-form solution for the bandwidth assignment problem. Then, the authors use an iterative algorithm to solve the other optimization issues.

Buyukates and Ulukus~\cite{buyukates2021timely_communication} focus on applications that use temporal data to predict something. For example, an application that uses the location and speed of users to avoid traffic jams when giving directions. In this application, the data recently produced has a bigger impact than the older ones. Thus, the authors select $m$ clients to participate in each communication round and make the server aggregates only the $k$ clients ($k < m$) with the earliest data. They also formulate the optimal $m$ and $k$ values given the total number of clients $n$ and present numerical results for $n = 100$.

In this work, we focus on scheduling Cross-Silo Federated Learning applications. In a Cross-Silo scenario, the clients are institutions, and they usually have more computational power and stabler network connection than Cross-Device clients. Thus, we assume that clients are available at all times and they all participate in each communication round. 

\section{Cross-Silo Federated Learning} \label{sec:related_work_cross_silo_fl}

Few papers focus on Cross-Silo Federated Learning to the best of our knowledge.

Rajendran~\etal~\cite{rajendran2021cloud} present a FL approach to predict the disease risk related to tobacco and radon. They use health care electronic record data as input and implement their approach using two different ML models, a neural network (NN) and a logistic regression (LR). They asynchronously trained both models, in which one institution trains the model at a time. The authors show the results in a simulated environment and a real-world scenario.

Huang~\etal~\cite{huang2021personalized_cross_silo} propose a method for Federated Learning focusing on training personalized models in each participating client. Instead of one unique global model, the FL server keeps a single model for each client and aggregates the weights of those participants whose models' weights are similar. The authors prove that their method improves the mean accuracy of all clients when there is no equal class distribution among all clients. Huang~\etal~\cite{huang2021personalized_cross_silo} conducted their experiments in a single machine and used four benchmark datasets.

Li~\etal~\cite{li2021federated} present an experimental study investigating the impact of different class distribution among clients in three different FL algorithms. In this study, they propose several data partitioning strategies. The authors created a benchmark dataset and concluded that there is no FL algorithm better in all scenarios. 
\section{Scheduling Distributed Machine Learning Jobs} \label{sec:related_work_scheduling_distributed_ml}

The majority of works focus on determining the optimal number of parameter servers and workers per job when scheduling multiple ML jobs in limited resources~\cite{zhang2017slaq, bao2018online_scheduling_distributed, zhang2020online_heterogeneous_distributed}. They assume that all workers will have the same amount of data and allocate them as close as possible. These two assumptions are the main difference from our work, where each client stores their heterogeneous private datasets in different cloud regions or even cloud providers. However, some recent papers consider stragglers~\cite{mohamadi2019distributed_ml_stragglers}, the network performance~\cite{liu2020distributed_ml_networks}, or locality awareness~\cite{yu2021distributed_ml_locality} being closer to ours.

Amiri~\etal~\cite{mohamadi2019distributed_ml_stragglers} consider transient stragglers among workers during the distributed ML training. Transient stragglers are workers with sporadic slowness due to temporary network disconnection, as an example. To handle them, the authors divide the central dataset into $n$ small chunks assuming that each worker will compute over a number of them sequentially. Then, the parameter server sends each piece to multiple workers and waits for $k$ results from different chunks, $k \leq n$. The authors present the proposed system model and theoretical analysis for the minimum average completion time. Finally, they explain two scheduling schemes for chunks assignment to the workers, and their experimental results present better completion time than other algorithms in the literature. One aspect of this work is the data exchange between the tasks, prohibitive in a Federated Learning scenario. Thus, the whole FL execution needs to consider stragglers' execution time.

Liu~\etal~\cite{liu2020distributed_ml_networks} focus on the impact of Optical Circuit Switches (OCSes) on multiple distributed ML training jobs execution in a data center or cluster. OCSes are energy-saving and high-performance switches that use light properties to make light passively flow in the desired direction. Hence, each port of an OCS switch only supports the communication to another port in a single way. If the application needs to send any message in another direction to another port, the OCS switch needs time to reconfigure itself. Thus, Liu~\etal~proposed two scheduling policies that consider the reconfiguration time. The Heaviest-Load-First (HLF) policy to schedule tasks within the same distributed ML job, and Shortest Weighted Remaining Time First (SWRT) to schedule different training interleaving their computation and communication phases. Besides handling possible network contention, the authors assume that all workers will have the same dataset size, class distribution and computational power, which is not always valid in a Federated Learning scenario due to privacy concerns.

Yu~\etal~\cite{yu2021distributed_ml_locality} formulate an optimization model to allocate tasks from different distributed ML jobs into a set of physical machines regarding resource and locality-aware constraints, named the offline distributed Machine Learning resource scheduling problem (DMLRS). DMLRS needs to know when each ML training job arrives and determines the best allocation scheme to all workers and parameter servers to each ML training job minimizing the communication time between them. They assume that the parameter server and the workers can co-locate in the same physical machine. They also consider that communication happens after training a few samples instead only at the end of a whole epoch. Besides, the authors propose an online scheduling algorithm based on a reformulation of DMLRS to a primal-dual and online problem. Despite presenting a locality-aware scheduling problem, this work has assumptions that cannot be valid in a Federated Learning scenario. First, they assume a central dataset, which is impossible in FL. Second, Yu~\etal~assume that the communication between workers and parameter server happens more frequently than in a FL scenario, where clients and the server communicate only after a few training epochs. Finally, the co-location of clients and servers in Federated Learning can help malicious clients discover other clients' information using reverse engineering on the weights updates~\cite{truong2021privacy_preservation_fl}. Thus, it is safer to allocate tasks to different resources in FL.

\section{Distributed Machine Learning and Federated Learning on Clouds} \label{sec:related_work_fl_ml_clouds}

Regarding the papers handling distributed Machine Learning on Clouds, most of them use cloud services as a tool to evaluate their scheduling proposal~\cite{mohamadi2019distributed_ml_stragglers, yu2021distributed_ml_locality} or to verify the central dataset integrity~\cite{zhao2020distributed_ml_integrity_verification}. We found few research papers that consider aspects of Cloud Computing to propose their solution~\cite{zhang2020machine_learning_volatile, duong_quang2018distributed_ml_iaas, duong2019fc2, wagenlander_2020_spotnik}. However, the authors assume the equal division of the central dataset among workers, and they usually use a single region to allocate all cloud resources. These facts reinforce that distributed ML do not concern about data privacy and heterogeneity, which are the essence of Federated Learning.

Zhang~\etal~\cite{zhang2020machine_learning_volatile} consider Spot (or preemptible) cloud instances to train distributed ML tasks. Cloud providers offer their spare capacity as preemptible instances with a huge discount, but they can revoke them at any time. As there is no guarantee that all workers from a distributed ML job will be available throughout the execution, Zhang~\etal study the convergence of classical algorithms to distributed ML training when the number of workers varies. They present a formula to obtain the optimal number of workers to deploy so that the algorithm does not diverge. They also validate their results using Amazon EC2~\cite{aws_ec2} Spot instances.

Duong and Quang~\cite{duong_quang2018distributed_ml_iaas, duong2019fc2} present a system to execute distributed ML jobs into on-demand instances of a cloud provider called  FC$^2$. They implement a simple web interface so that ML practitioners add their ML model characteristics and available budget, and FC$^2$ calculates the total number of workers to deploy into different instance types from a pool of available ones. The authors also implement two heuristics to recommend the instances, one considering the execution time per instance and the other the instances' bandwidth. Doung and Quang execute all results using Amazon EC2~\cite{aws_ec2} instances.

Wagenländer~\etal~\cite{wagenlander_2020_spotnik} propose Spotnik to deal with instance revocations due to preemptible cloud instances in distributed ML training. They assume a decentralized training approach in which the workers communicate with each other in a pre-defined ring pattern to aggregate their results. Thus, in the communication phase, if a worker $w_i$ cannot reach its neighbor $w_j$, it assumes a revocation occurred, ignores the changes in the current iteration, removes $w_j$ from the known topology, and propagates this change. Spotnik also adapts its training method accordingly to the current number of workers. If the number of workers is low, Spotnik uses synchronous strategies to calculate the aggregated results and, if the number of workers is high, Spotnik uses asynchronous ones.

To the best of our knowledge, few works tackle the problem of federated learning on clouds in the related literature. 

Liu~\etal~\cite{liu2020client} present a hierarchical FL architecture with mobile devices as clients. Their principle idea is the addition of an edge layer of servers. These edge servers aggregate the results of a fraction of the clients and send their aggregation to a central cloud server. Then, this central server aggregates the results of all edge servers and, consequently, all clients. The authors present the algorithm to this architecture and its convergence analysis in the paper. However, they only show simulation results to prove their convergence analysis.

Fang~\etal~\cite{FANG2020101889} propose an architecture for Federated Learning in the cloud focusing on privacy. Their architecture consists of a central server on the cloud with clients that uses ElGamal encryption~\cite{crypt_elgaman} to encrypt all messages. They present how the server and clients exchange their encryption keys and how the framework works. The authors compare their solution theoretically with other privacy-concerning deep learning methods. Besides, they simulate the FL environment in a local machine and present the accuracy, execution times, and messages size of each one.

The only found work that runs a FL approach in a cloud environment is the work of Rajendran~\etal~\cite{rajendran2021cloud}. They presented the results of both implemented models in a scenario with two clients in a simulated environment and on the Microsoft Azure Cloud Databricks~\cite{azure_databricks}, an open-source tool for data engineering and collaborative data science, to exchange the ML model between two institutions.

In this work, we focus on synchronous FL training on VMs in the cloud and how we can schedule each actor (the server and clients) to minimize the total execution costs respecting the location of each client's dataset. 


\section{Summary}


As presented in this chapter, most work on Federated Learning in the literature tackles the clients' unstable network from the Cross-Device architecture. In this scenario, the server needs to sample a fraction of clients in each communication round, as there are usually hundreds or thousands of devices connected. We focus on Cross-Silo FL, which assumes fewer clients and a better network connection in the present work. The clients are dedicated machines or clusters, and the server usually samples all to participate in each round as they are available throughout the entire execution. Moreover, we intend to create a generic Cross-Silo FL scheduler and, thus, we cannot take advantage of algorithms that focus on CNNs or RNNs. 

Thus, Table \ref{tab:papers_fl} presents all previously described works regarding Federated Learning compared to ours. We describe the ML algorithm that each work implements (ML model), whether the authors evaluated their proposal using simulation or real-world schemes (Environment), and the FL type the paper focus. For the papers proposing scheduling solutions, we also present the minimization objective and the criteria used in their solution. If the authors do not mention which ML model they focus on, we use the N/S value.

\begin{table}[htbp]
\caption{Recent work on Federated Learning research area} \label{tab:papers_fl}
\begin{center}
\tiny
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Paper} & \textbf{ML model} & \textbf{Environment} & \textbf{FL type} & \begin{tabular}[c]{@{}c@{}}\textbf{Minimization} \\ \textbf{Objective} \end{tabular} & \textbf{Criteria} \\
\hline
Li~\etal~\cite{li2018federated} & LR and RNNs & Simulation & Cross-Device & - & - \\
\hline
Ji~\etal~\cite{shaoxing2019learning_attentive} & RNNs & Simulation & Cross-Device & - & - \\
\hline
Xu~\etal~\cite{jinijn2020ternary_compression} & CNNs & Simulation & Cross-Device & - & - \\
\hline
Chen~\etal~\cite{chen2020layerwise} & DNNs & Simulation & Cross-Device & - & - \\
\hline
Liu~\etal~\cite{liu2020client} & CNNs & Simulation & Cross-Device & - & - \\
\hline
Fang~\etal~\cite{FANG2020101889} & CNNs & Simulation & Cross-Device & - & - \\
\hline
Yang~\etal~\cite{yang2020scheduling} & N/S & Simulation & Cross-Device & Communication costs & Clients' response time \\
\hline
Xia~\etal~\cite{xia2020multi_armed_scheduling} & LR & Simulation & Cross-Device & Total time & No previous knowledge \\
\hline
Ren~\etal~\cite{ren2021joint_resource_allocation} & Any & Simulation & Cross-Device & \begin{tabular}[c]{@{}c@{}} System and learning \\ costs \end{tabular} & \begin{tabular}[c]{@{}c@{}}Computation frequency,\\bandwidth, subcarrier\\allocation and transmission\\ power\end{tabular} \\
\hline
\begin{tabular}[c]{@{}c@{}}Buyukates and\\Ulukus~\cite{buyukates2021timely_communication}\end{tabular} & N/S & Simulation & Cross-Device & \begin{tabular}[c]{@{}c@{}} Usage delay of clients' \\ data \end{tabular} & \begin{tabular}[c]{@{}c@{}}Limited communication\\resources and client\\availability \end{tabular} \\
\hline
Huang~\etal~\cite{huang2021personalized_cross_silo} & DNNs & Simulation & Cross-Silo & - & - \\
\hline
Li~\etal~\cite{li2021federated} & CNNs & Simulation & Cross-Silo & - & - \\
\hline
Rajendran~\etal~\cite{rajendran2021cloud} & NN and LR & Single-cloud & Cross-Silo & - & - \\
\hline
Our work & DNNs & Multi-cloud & Cross-Silo & \begin{tabular}[c]{@{}c@{}} Execution time \\ and costs \end{tabular} & \begin{tabular}[c]{@{}c@{}} Clients' dataset locality, \\ communication and training time \end{tabular} \\
\hline
\end{tabular}
\end{center}
\end{table}

Regarding the presented works on scheduling distributed Machine Learning (DML) jobs, they focus on three aspects that our scheduler could consider: non-persistent stragglers~\cite{mohamadi2019distributed_ml_stragglers}, network performance~\cite{liu2020distributed_ml_networks}, and locality of the dataset and tasks~\cite{yu2021distributed_ml_locality}. Table \ref{tab:papers_distributed_ml} compares these works presenting their main characteristics. We present the minimization objective of each paper, how the authors solved their optimization problem (Solution), in which environment they tested the solution, and if the authors considered an online or offline problem. An online optimization problem is when new tasks can arrive during the execution, and, in the offline approach, all tasks' information is already available before the scheduling.


\begin{table}[htbp]
\caption{Recent work on scheduling Distributed Machine Learning (DML) jobs} \label{tab:papers_distributed_ml}
\begin{center}
\tiny
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Paper} & \begin{tabular}[c]{@{}c@{}}\textbf{Minimization}\\\textbf{Objective} \end{tabular} & \textbf{Solution} & \textbf{Environment} & \begin{tabular}[c]{@{}c@{}} \textbf{Problem} \end{tabular} \\
\hline
Amiri~\etal~\cite{mohamadi2019distributed_ml_stragglers} & \begin{tabular}[c]{@{}c@{}} Total delay in\\a single DML job \end{tabular} & \begin{tabular}[c]{@{}c@{}} Two exact task scheduling schemes \end{tabular} & AWS (Amazon EC2) & Offline \\
\hline
Liu~\etal~\cite{liu2020distributed_ml_networks} & \begin{tabular}[c]{@{}c@{}}Total weighted job computation\\time of multiple DML jobs\end{tabular} & \begin{tabular}[c]{@{}c@{}} Two heuristics (one focus on intra-job\\and another on inter-job scheduling) \end{tabular} & Physical cluster & Online \\
\hline
% Yu~\etal~\cite{yu2021distributed_ml_locality} & \begin{tabular}[c]{@{}c@{}} Maximize one metric based\\on job completion time\\(\eg, fairness)\end{tabular} & \begin{tabular}[c]{@{}c@{}} Approximation algorithm\\based on randomized rounding \end{tabular} & Physical cluster & Online \\
Yu~\etal~\cite{yu2021distributed_ml_locality} & \begin{tabular}[c]{@{}c@{}} Maximize fairness of multiple\\DML jobs\end{tabular} & \begin{tabular}[c]{@{}c@{}} Approximation algorithm\\based on randomized rounding \end{tabular} & Physical cluster & Online \\
\hline
\end{tabular}
\end{center}
\end{table}

==> old_articles/sbac_text.tex <==
\begin{abstract}
Under the coordination of a central server, Federate Learning (FL) enables a set of clients to collaboratively train a global machine learning model without exchanging their local data. When such clients have powerful machines, it is called cross-silo FL, and they store their data in private repositories denoted silos. We are interested in this paper in cross-silo FL where silos are geographically located in different regions of multi-cloud providers. Thus, aiming at minimizing financial costs and execution times of a cross-silo FL application, we propose a model based on a scheduling problem mathematical formulation, which receives as input both the application parameters and the cloud providers' resource features where clients' data are stored and renders the best assignment of clients and server to virtual machines. This formulation is part of a framework proposal to execute FL applications in different cloud providers.
Taking as a use case a Tumor-Infiltrating Lymphocytes Classification problem, an FL application whose clients' datasets spread over different cloud providers' data repositories, evaluation results show that our model is scalable and improves the execution time and financial costs of the FL application by up to 53.70\% and 48.34\% in a scenario with 50 clients, executing in around 200 seconds, when compared to results where VMs are randomly selected. Experimental results with client silos in different Google (GCP) and Amazon (AWS) cloud regions also confirmed the effectiveness of our proposed model in a real multi-cloud environment.
\end{abstract}

\begin{IEEEkeywords}
Scheduling Problem, Federated Learning, Multi-Cloud
\end{IEEEkeywords}

\section{Introduction}

Proposed by McMahan~\etal~\cite{mcmahan2017communication}, Federated Learning (FL) is an emerging distributed Machine Learning (ML) technique where the participants (clients) collaboratively train a ML model without sharing their respective private data~\cite{shen2021difference_distributed_federated_learning}. Under the coordination of a central server, each client trains the model locally and communicates only the model weights to the server that, in its turn, updates its global model. Federated Learning has received much attention during the past few years due to the increasing concern with data privacy, particularly with current data protection laws (\eg, GPDR\footnote{https://gdpr-info.eu/} in Europe).

The client-server architecture of FL, also called Model-Centric Federated Learning~\cite{yang2019federated}, can be classified into Cross-Device or Cross-Silo Federated Learning. The former has low-powered clients, such as mobile phones~\cite{mcmahan2017communication}, while the latter has few clients (\eg, companies, institutions, hospitals~\cite{rajendran2021cloud}) with private large dataset repositories, denoted silos. 

This work focuses on Cross-Silo Federated Learning, also taking into account that, due to datasets gradually growing~\cite{villars2011big}, many clients keep their silos in cloud storage repositories~\cite{huan2013big_data_storage, leavitt2013storage} which offer data privacy guarantees and availability. In such a context, we also consider that client silos can be stored in different cloud providers (\eg~Amazon (AWS) S3, Google Cloud (GCP) Storage, etc.). Moreover, the physical infrastructure of a cloud provider is usually divided into independent and isolated geographic regions~\cite{aws_regions_zones, gcp_regions_zones}, each of them offering several types of virtual machines with different performance and financial costs. Consequently, a multi-cloud platform offers multiple choices of virtual machine types, regions, and cloud providers, with different execution and communication times and costs, for executing the clients and the server of an FL application. 

Therefore, considering different types, regions, and cloud providers, the question is how to select the best set of virtual machines to execute the clients and the server of an FL application, whose datasets were previously allocated in one or more storage systems of one of the cloud providers, minimizing both the execution time and the financial cost of the FL application. In order to solve this scheduling problem, we propose in this paper a mathematical formulation model which receives as input information about the FL application as well as about the multi-cloud environment and provides a weighted optimization function whose aim is to minimize the conflicting objectives cost and time. Our mathematical model is part of a framework proposal to execute FL applications in a multi-cloud environment, aiming to minimize time and costs while keeping data privacy.

This framework receives as input information concerning the FL application (e.g. number of clients, location of each client dataset, number of communication rounds, etc) and the environment (e.g., number of CPUs and GPUs in each VM, the price of each VM in each region, limits of VMs per region, etc) and outputs a scheduling map. It also deploys the selected VMs and starts the tasks following the obtained map.

The model has been evaluated theoretically and in a multi-cloud platform with AWS and GCP. To this end, we chose a use-case application, which searches for Tumor-Infiltrating Lymphocytes (TILs) in high-resolution scanned human tissue images aiming to understand the patient's cancer extension and predicting the most suitable treatments. 

Experiments with different data placement scenarios of such an application have been conducted for evaluating the scalability of the model, its effectiveness when compared to a random user VM selection, and its accuracy when compared to a real multi-cloud environment with a client's silo in either Google Cloud Storage or AWS S3 of different regions. 

The paper is organized as follows. Section \ref{sec:relworks} introduces related work. Section \ref{sec:formula} presents our mathematical formulation to the problem of scheduling FL clients and the server to a multi-cloud environment. Section \ref{sec:problem_description} and Section \ref{sec:flower} briefly describe the use-case application and Flower, a tool that creates FL systems. Section \ref{sec:results} presents and discusses experimental evaluation results. Finally, Section \ref{sec:conclusions} concludes the paper and proposes some future work.

\section{Related work}
\label{sec:relworks}

Most existing Federated Learning works tackle Cross-Device architectures, where the server samples a fraction of clients in each communication round, among hundreds or thousands of connected devices \cite{ren2021joint_resource_allocation, buyukates2021timely_communication}, while few of them focus on Cross-Silo Federated Learning \cite{rajendran2021cloud, huang2021personalized_cross_silo, li2021federated}. However, to the best of our knowledge, none of the latter consider the scheduling problem of FL clients and the server in a cloud or datacenter environment. 

Regarding distributed machine learning in general, a majority of works focus on the job scheduling problem of multiple ML jobs that should be allocated among a number of limited resources~\cite{zhang2020online_heterogeneous_distributed, liu2020distributed_ml_networks, yu2021distributed_ml_locality}. Few of them handle the scheduling problem of a unique distributed ML application. In~\cite{mohamadi2019distributed_ml_stragglers}, Amiri~\etal~consider that some tasks (called workers) may present sporadic slowness due, for instance, to temporary network disconnection. To overcome such a problem, the central dataset is divided into small $n$ chunks. Each worker should then compute a number of them sequentially. Thus, a server task sends chunks to multiple workers and waits for $k$ results, $k \leq n$. The authors propose two scheduling schemes for chunks assignment to the workers aiming at minimizing the average completion time. However, the data-sharing approach to this problem is not suitable for Federated Learning scenarios where data privacy and heterogeneity are essential concerns. 

\section{Scheduling FL Clients and Server to a Multi-Cloud Environment} \label{sec:formula}

In this section, we present our application and multi-cloud models. Then, we describe our mathematical formulation to schedule FL clients and server into a multi-cloud environment.

\subsection{FL application Model} \label{subsec:FLappmodel}

An FL application is a distributed algorithm, composed of a set of clients, $C$, and a server, $s$, that uses communication barriers along execution. We consider in this work, that the FL application executes a set of rounds, each one divided into five steps. In the first one, the server sends the message $s\_msg_{train}$ containing the model weights to all clients. After receiving the weights, in Step 2, each client, $c_i \in C$, trains the neural network for a fixed number of epochs on the local training dataset and sends the updates back to the server, through the message $c\_msg_{train}$. Then, in Step 3, the server receives all updates, aggregates them, and sends the final weights to the clients ($s\_msg_{aggreg}$ message). Upon reception, in Step 4, each client updates their respective weights, tests the model with the test dataset, and sends its evaluation metrics (for example, accuracy and precision) to the server in the message $c\_msg_{test}$. Finally, in Step 5, the server aggregates the evaluation metrics of all clients to have the global metrics. Figure \ref{fig:fl_round} shows the execution steps of a round.
%
\begin{figure}[htbp]
 \centering
 \includegraphics[width=0.55\columnwidth]{images/FL_round.pdf}
 \caption{Steps of one round of a Federated Learning Application}
 \label{fig:fl_round}
\end{figure}

\subsection{Multi-Cloud Model} \label{subsec:multcloud}

Usually, commercial clouds have their physical infrastructures spread in different regions, which are independent and isolated geographically. For instance, there are currently 26 regions in AWS~\cite{aws_regions_zones} and 34 regions in GCP~\cite{gcp_regions_zones}.

Each region offers computational resources packaged as Virtual Machines (VMs). Each VM has a number of virtual cores, named virtual CPUs (vCPUs), and may have one or more Graphics Processing Units (GPUs) connected to it. Thus, let $P$ be a set of available cloud providers. A provider $p_{j} \in P$ has associated to it a set of regions $R_{j}$ and a fixed cost $cost\_t_{j}$ (in \$ per GB) to send any message from itself to any other VM, inside or outside the provider, as observed experimentally. A provider $p_j$ usually offers a limited number of GPUs ($N\_GPU_{j}$) and vCPUs ($N\_CPU_{j}$). Moreover, in each region $r_{jk} \in R_{j}$, the number of available GPUs and vCPUs are bounded ($N\_L\_GPU_{jk}$ and $N\_L\_CPU_{jk}$, respectively). 

Yet, each region $r_{jk} \in R_{j}$ has a set of available VM instance types, $V_{jk}$, that can be deployed in it, where each $vm_{jkl} \in V_{jk}$ contains a number of vCPUs, $cpu_{jkl}$ and a number of GPUs, $gpu_{jkl}$, with a fixed hiring cost (in \$ per second) $cost_{jkl}$. 

\subsection{Mathematical Formulation}

The problem of scheduling tasks in distributed computing resources is an NP-complete one~\cite{ullman1975np}, even in simple scenarios. Furthermore, some features of multi-clouds render it more difficult. Thus, we model our scheduling problem as a Mixed-Integer Linear Programming problem. In our scheduling problem, we have two objectives: minimize the monetary cost and the total execution time (makespan) of the application. Here, we also consider that the obtained solution has to respect the constraints of a deadline, named $T$, and of a budget, called $B$, given by the user. 

Considering that the FL application executes $n\_rounds$, each one for a similar amount of time, we can divide $B$ and $T$ by $n\_rounds$ to obtain the maximum budget and deadline for a single FL round, named $B_{round}$ and $T_{round}$, respectively. Hence, we formulate the scheduling problem for one round.

Table \ref{tab:var} presents the notation and variables used in the mathematical formulation. The proposed objective function (Equation \ref{eq:obj}) is a weighted function that minimizes the monetary cost, $total\_costs$, and the makespan, $t_m$, of a single FL round, where $\alpha$, ranging from zero to one, is the weight given by the user for the objectives. Usually, once those objectives are conflicting, they cannot reach the optimal values simultaneously. For instance, for $\alpha$ values close to 1, the formulation prioritizes low costs solutions rather than small makespans. On the other hand, when $\alpha = 0.5$, both objectives receive the same importance.
%
\begin{table*}
\caption{Notation and variables used.} \label{tab:var}
\begin{center}
\begin{tabular}{|r|l|}
\hline
\textbf{Name} & \textbf{Description} \\
\hline
$C$ & Set of clients in the FL application \\
\hline
$P$ & Set of available cloud providers \\
\hline
$p_{j}$ & A cloud provider \\
\hline
$R_{j}$ & Set of regions available in provider $p_j$ \\
\hline
$r_{jk}$ & A region of provider $p_{j}$ \\ 
\hline
$V_{jk}$ & Set of instance types available in region $r_{jk}$ \\
\hline
$vm_{jkl}$ & A instance type of region $r_{jk}$ \\
\hline
$B_{round}$ & Maximum budget to a single FL round \\
\hline
$T_{round}$ & Maximum deadline to a single FL round \\
\hline
$T_{max}$ & Maximum time of a single FL round \\
\hline
$N\_GPU_{j}$ & Maximum number of available GPUs in the provider $p_{j}$ \\
\hline
$N\_CPU_{j}$ & Maximum number of available vCPUs in the provider $p_{j}$ \\
\hline
$cost\_t_{j}$ & Cost (in \$ per GB) of sending a message from provider $p_{j}$ \\
\hline
$N\_L\_GPU_{jk}$ & Maximum number of available GPUs in region $r_{jk}$ \\
\hline
$N\_L\_CPU_{jk}$ & Maximum number of available vCPUs in region $r_{jk}$ \\
\hline
$cpu_{jkl}$ & Number of vCPUs in the instance type $vm_{jkl}$ \\
\hline
$gpu_{jkl}$ & Number of GPUs in the instance type $vm_{jkl}$ \\
\hline
$cost_{jkl}$ & Cost (in \$ per second) of instance type $vm_{jkl}$ \\
\hline
$c_{i}$ & A client of the FL application \\
\hline
$size(s\_msg_{train})$ & Size of training message sent by the server to a client \\
\hline
$size(s\_msg_{aggreg})$ & Size of test message sent by the server to a client \\
\hline
$size(c\_msg_{train})$ & Size of training message sent by a client to the server \\
\hline
$size(c\_msg_{test})$ & Size of test message sent by a client to the server \\
\hline
$total\_costs$ & Total financial costs of a single FL round \\
\hline
$t_{m}$ & Total execution time (makespan) of a FL round \\
\hline
$t\_exec_{ijkl}$ & Computational time (training and test) of client $c$ in $vm_{jkl}$ \\
\hline
$t\_comm_{jklm}$ & Communication time (training and test messages) between region $r_{jk}$ and region $r_{lm}$ \\
\hline
$t\_aggreg_{jkl}$ & Aggregation time of server in $vm_{jkl}$ \\
\hline
$vm\_costs$ & Total financial cost of all VMs in a single FL round \\
\hline
$comm\_costs$ & Total financial cost of message exchange within a FL round \\
\hline
$x_{ijkl}$ & Binary variable which indicates if client $c_{i}$ executes on $vm_{jkl}$ or not \\
\hline
$y_{jkl}$ & Binary variable which indicates if the server executes on $vm_{jkl}$ or not \\
\hline
$\alpha$ & Weight given by the user for the objectives (ranging from 0 to 1) \\
\hline
\end{tabular}
\label{tab1}
\end{center}
\end{table*}
%
\begin{equation}
 \min \alpha \times total\_costs + ( 1 - \alpha) \times t_m \label{eq:obj}
\end{equation}

Let the binary variables $x_{ijkl}$ indicate whether a client $c_i$ will execute on VM $vm_{jkl}$ of region $r_{jk}$ of provider $p_j$ ($x_{ijkl} = 1$), or not ($x_{ijkl} = 0$), and let $y_{jkl}$ be the analogous representation for the server $s$. The variable $total\_costs$ includes the VMs' execution costs ($vm\_costs$), computed as Equation \ref{eq:vm_costs}, and the message transfer costs ($comm\_costs$), described in Equation \ref{eq:transfer_costs}, where $comm_{jm}$, presented in Equation \ref{eq:comm}, is the cost to exchange the FL messages between provider $p_{j}$ and $p_{m}$ ($j$ can be equal to $m$). Therefore, $total\_costs$ is calculated as in Equation \ref{eq:total_costs}.
%
\begin{multline}
\resizebox{0.90\hsize}{!}{$vm\_costs = \sum_{c_i \in C}\sum_{p_j \in P}\sum_{r_{jk} \in R_{j}}\sum_{vm_{jkl} \in V_{jk}}(x_{ijkl} \times cost_{jkl}$} \\
\resizebox{0.90\hsize}{!}{$\times t_{m}) \  + \sum_{p_{j} \in P}{\sum_{r_{jk} \in R_{j}}\sum_{vm_{jkl} \in V_{jk}}(y_{jkl} \times cost_{jkl} \times t_m)}$} \label{eq:vm_costs}
\end{multline}
%
\begin{multline}
\resizebox{0.95\hsize}{!}{$comm\_costs = \sum_{c_i \in C}\sum_{p_{j} \in P}\sum_{r_{jk} \in R_{j}}\sum_{vm_{jkl} \in V_{jk}} \sum_{p_{m} \in P}\sum_{r_{mn} \in R_{m}}$} \\
\resizebox{0.55\hsize}{!}{$\sum_{vm_{mno} \in V_{mn}}(x_{ijkl} \times y_{mno} \times comm_{jm})$} \label{eq:transfer_costs}
\end{multline}
%
\begin{multline}
\resizebox{0.89\hsize}{!}{$comm_{jm} = (size(s\_msg_{train}) + size(s\_msg_{aggreg}))\times cost\_t_{m}$}\\
\resizebox{0.70\hsize}{!}{$ + (size(c\_msg_{train})\  + size(c\_msg_{test})) \times cost\_t_{j}$} \label{eq:comm}
\end{multline}
%
\begin{equation}
 total\_costs = vm\_costs + comm\_costs \label{eq:total_costs}
\end{equation}

Both the monetary cost and the makespan have to be first normalized. The normalization procedure updates the target values to share the same minimum and maximum values. Thus, $total\_costs$ is divided by the product of the monetary cost of hiring the most expensive VM, the maximum execution time of an FL round ($T_{max}$), and the number of tasks (clients and server); plus the product of the most expensive message exchange between providers ($comm_{jm}$) and the number of clients, as shown in Equation \ref{cost_norm}. Similarly, the makespan is divided by the maximum execution time of a FL round ($T_{max}$).
%
\begin{multline}
\max_{p_{j} \in P, r_{jk} \in R_{j}, vm_{jkl} \in V_{jk}} (cost_{jkl}) \times T_{max} \times (|C| + 1)\\
+ \max_{p_j, p_m \in P} (comm_{jm}) \times |C| \label{cost_norm}
\end{multline}

The objective function is subject to the following constraints. 
Constraints \ref{r1} and \ref{r2} guarantee that the 
%given 
budget and deadline for a FL application round are not violated, while constraints \ref{r3} and \ref{r4} ensure that every client and the server execute on a single VM $vm_{jkl} \in V_{jk}$ in a region $r_{jk} \in R_{j}$ of a provider $p_{j} \in P$.
%
\begin{align}
& total\_costs \leq B_{round} \label{r1}
\end{align}
%
\begin{align}
& t_m \leq T_{round} \label{r2}
\end{align}
%
\begin{align}
& \resizebox{0.70\hsize}{!}{$\sum_{p_{j} \in P}{\sum_{r_{jk} \in R_{j}}{\sum_{vm_{jkl} \in V_{jk}} x_{ijkl}}} = 1 , \forall c_{i} \in C$} \label{r3}
\end{align}
%
\begin{align}
& \resizebox{0.60\hsize}{!}{$\sum_{p_{j} \in P}{\sum_{r_{jk} \in R_{j}}\sum_{vm_{jkl} \in V_{jk}} {y_{jkl}}} = 1$} \label{r4}
\end{align}

Constraints \ref{r5} to \ref{r8} guarantee that the solution will not exceed the maximum number of GPUs and vCPUs of each provider. Constraints \ref{r5} ensure that the total number of available GPUs does not exceed the global limit, while constraints \ref{r6} limit the total number of available vCPUs in each provider. Constraint \ref{r7} has the same meaning as \ref{r5}, but here the GPU limit is by region. Constraint \ref{r8} is the vCPUs limit constraints per region, similarly as Constraint \ref{r6}.
% 
\begin{multline}
\resizebox{0.95\hsize}{!}{$\sum_{c_{i} \in C}{\sum_{r_{jk} \in R_j}{\sum_{vm_{jkl} \in V_{jk}} x_{ijkl} \times gpu_{jkl}}} + \sum_{r_{jk} \in R_j}\sum_{vm_{jkl} \in V_{jk}}(y_{jkl}$} \\
\resizebox{0.40\hsize}{!}{$\times gpu_{jkl}) \leq N\_GPU_j , \forall p_{j} \in P$} \label{r5}
\end{multline}
%
\begin{multline}
\resizebox{0.95\hsize}{!}{$\sum_{c_{i} \in C}{\sum_{r_{jk} \in R_j}{\sum_{vm_{jkl} \in V_{jk}} x_{ijkl} \times cpu_{jkl}}} +\sum_{r_{jk} \in R_j}\sum_{vm_{jkl} \in V_{jk}}(y_{jkl}$} \\
\resizebox{0.40\hsize}{!}{$\times cpu_{jkl}) \leq N\_CPU_j , \forall p_{j} \in P$} \label{r6}
\end{multline}
%
\begin{multline}
\resizebox{0.95\hsize}{!}{$\sum_{c_{i} \in C}{\sum_{vm_{jkl} \in V_{jk}}{x_{ijkl} \times gpu_{jkl}}} \ + \sum_{vm_{jkl} \in V_{jk}}{y_{jkl} \times gpu_{jkl}}$} \\
\resizebox{0.50\hsize}{!}{$\leq N\_L\_GPU_{jl} , \ \forall p_{j} \in P, \forall r_{jk} \in R_{j}$} \label{r7}
\end{multline}
%
\begin{multline}
\resizebox{0.95\hsize}{!}{$\sum_{c_{i} \in C}{\sum_{vm_{jkl} \in V_{jk}}{x_{ijkl} \times cpu_{jkl}}} \ + \sum_{vm_{jkl} \in V_{jk}}{y_{jkl} \times cpu_{jkl}}$} \\
\resizebox{0.50\hsize}{!}{$\leq N\_L\_CPU_{jl} , \ \forall p_{j} \in P, \forall r_{jk} \in R_{j}$} \label{r8}
\end{multline}

Next, constraint \ref{r9} guarantees that the FL application will finish before $t_m$, which is considered as the makespan of the FL round. Finally, constraints \ref{r10} and \ref{r11} define the domain of the decision variables $x_{ijkl}$ and $y_{jkl}$, respectively.
%
\begin{multline}
x_{ijkl} \times y_{mno} \times (t\_exec_{ijkl} + t\_comm_{jkmn} + t\_aggreg_{mno}) \\ 
\leq t_{m}, \forall c_{i} \in C, \forall p_{j},p_{m} \in P, \forall r_{jk} \in R_{j}, \forall vm_{jkl} \in V_{jk},\\
\forall r_{mn} \in R_{m},\  \forall vm_{mno} \in V_{mn} \label{r9}
\end{multline}
%
% \begin{multline}
% x_{ijkl} \in \{0, 1\},\forall c_{i} \in C,\forall p_{j} \in P,\forall r_{jk} \in R_{j},\\
% \forall vm_{jkl} \in V_{jk} \label{r10}
% \end{multline}
\begin{equation}
\resizebox{0.88\hsize}{!}{$x_{ijkl} \in \{0, 1\},\forall c_{i} \in C,\forall p_{j} \in P,\forall r_{jk} \in R_{j},\forall vm_{jkl} \in V_{jk}$} \label{r10}
\end{equation}
%
\begin{align}
\resizebox{0.70\hsize}{!}{$y_{jkl} \in \{0, 1\},\forall p_{j} \in P,\forall r_{jk} \in R_{j}, \forall vm_{jkl} \in V_{jk}$} & \label{r11}
\end{align}

\section{Case Study: Tumor-Infiltrating Lymphocytes Classification} \label{sec:problem_description}
%
The selected use-case application searches for Tumor-Infiltrating Lymphocytes (TILs) in high-resolution scanned human tissue images and creates maps representing their spatial distribution. However, the Whole Slide Tissue Images (WSIs) of scanned tissue can have up to 100K$\times$100K pixels, making it difficult for an expert to extract information from thousands of WSIs available in research studies. Because of that, Saltz \etal~\cite{saltz:2018} developed a deep learning application to classify and analyze TIL patterns from tissue images. 

For the evaluation of our proposal, we focus on the CNN training, which is one step of the application. We assume that the WSIs are previously divided into patches and classified by an expert. The centralized version of the CNN training in this TIL classification problem implements the VGG16 model~\cite{vgg_paper}, which has an input layer of size $224\times224\times3$. After this layer, the model has several convolutional and fully connected layers, ending with an output layer that determines if the TIL is positive or negative. The centralized version was implemented with the TensorFlow API~\cite{tensorflow2015-whitepaper}, which optimizes dataset readings by using multiple threads to load the images from the main memory and transfer them to the GPU memory.

\section{Federated learning using the Flower Framework} \label{sec:flower}

We used the Flower framework, proposed by Beutel \etal~\cite{beutel2021flower}, to build our federated learning system. Flower offers facilities to execute FL experiments, considering heterogeneous clients on simulation and real-world scenarios. It supports different ML frameworks underneath it (e.g., TensorFlow, PyTorch, or a custom one). The FL client implements the VGG16 model~\cite{vgg_paper}, using the TensorFlow API~\cite{tensorflow2015-whitepaper}.

For the aggregation function to the server, we chose the FedAvg~\cite{mcmahan2017communication} since it is already implemented in Flower and gives good results on different unbalanced schemes, as shown in Li~\etal~\cite{li2021federated}. FedAvg computes the weighted average from all clients using their respective dataset size as associated weight.

\section{Performance Evaluation} \label{sec:results}
%
\begin{table*}[t]
\caption{Instance types selected} \label{tab:setup}
\footnotesize
\begin{center}
\begin{tabular}{|c|c|l|c|c|c|c|c|c|}
\hline
Prov. & Region & \multicolumn{1}{c|}{VM} & vCPUS & \begin{tabular}[c]{@{}c@{}}RAM\\(GB)\end{tabular} & GPU & \begin{tabular}[c]{@{}c@{}}GPU\\memory (GB)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Costs per\\hour (\$)\end{tabular} & ID \\ \hline
\multirow{6}{*}{AWS} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}N. Virginia\\ (us-east-1)\end{tabular}} & \textit{g4dn.2xlarge} & 8 & 32 & Nvidia Tesla T4 Tensor Core & 16 & 0.7520 & $vm_{111}$ \\
\cline{3-9} 
 & & \textit{g3.4xlarge} & 16 & 122 & Nvidia Tesla M60 & 8 & 1.1400 & $vm_{112}$ \\ 
\cline{3-9}
 & & \textit{t2.xlarge} & 4 & 16 & - & - & 0.1856 & $vm_{113}$ \\
\cline{2-9} 
\cline{2-9} 
 & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Oregon\\ (us-west-2)\end{tabular}} & \textit{g4dn.2xlarge} & 8 & 32 & Nvidia Tesla T4 Tensor Core & 16 & 0.7520 & $vm_{121}$ \\
\cline{3-9} 
 & & \textit{g3.4xlarge} & 16 & 122 & Nvidia Tesla M60 & 8 & 1.1400 & $vm_{122}$ \\
\cline{3-9}
 & & \textit{t2.xlarge} & 4 & 16 & - & - & 0.1856 & $vm_{123}$ \\
\hline
\hline
\multirow{7}{*}{GCP} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Iowa\\ (us-central1)\end{tabular}} & \textit{n1-standard-8} with Turing GPU & 8 & 30 & Nvidia Tesla T4 Tensor Core & 16 & 0.7300 & $vm_{211}$ \\ 
\cline{3-9} 
 & & \textit{n1-standard-16} with Pascal GPU & 16 & 60 & Nvidia Testa P4 & 8 & 1.3600 & $vm_{212}$ \\
\cline{3-9} 
 & & \textit{n1-standard-8} with Volta GPU & 8 & 30 & Nvidia V100 Tensor Core & 16 & 2.8600 & $vm_{213}$ \\
\cline{3-9}
 & & \textit{e2-standard-4} & 4 & 16 & - & - & 0.1340 & $vm_{214}$ \\
\cline{2-9}
\cline{2-9} 
 & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Oregon\\ (us-west1)\end{tabular}} & \textit{n1-standard-8} with Turing GPU & 8 & 30 & Nvidia Tesla T4 Tensor Core & 16 & 0.7300 & $vm_{221}$ \\
\cline{3-9} 
 & & \textit{n1-standard-8} with Volta GPU & 8 & 30 & Nvidia V100 Tensor Core & 16 & 2.8600 & $vm_{222}$ \\
\cline{3-9}
 & & \textit{e2-standard-4} & 4 & 16 & - & - & 0.1340 & $vm_{223}$ \\
\hline
\end{tabular}
\end{center}
\end{table*}

For our experiments, we considered Amazon Web Services (AWS) and Google Cloud Provider (GCP) as cloud providers with two regions at each of them: N. Virginia (\textit{us-east-1}) and Oregon (\textit{us-west-2}) regions in AWS; and Iowa (\textit{us-central1}) and Oregon (\textit{us-west1}) regions in GCP. 

Initially, we planned to have a testbed composed of several VMs with GPU in both AWS and in GCP, varying from the Kepler GPU architecture to the Ampere one. However, the CUDA version 10.0, used by the use-case TILs application, is not compatible with either of these two architectures. Consequently, we had to discard such GPU architectures from our testbed. Furthermore, experiments showed that a VM with the Volta GPU in AWS had constantly higher execution times than with the Turing one, which led us to also discard the former from our testbed, due to its unexpected behaviour. Finally, in other experiments, we observed that it was not possible to allocate, in either of the two regions, some types of GPU architectures in GCP. Thus, such GPUs were not taken into account either.

Hence, considering all the above constraints, for each region in AWS, we selected two instance types with GPU, Maxwell and Turing, and one instance without GPU. For GCP, we chose instances from the general-purpose N1 family with the same number of vCPUs as the AWS counterparts. Each instance had one GPU, Pascal, Turing or Volta, attached to it. Additionally, we also selected an instance without GPU. Note that in GCP, some GPU architectures are not available in all regions, thus, the number of instance types varies for each region. 

Table \ref{tab:setup} summarizes our VM instance selection in both platforms, giving also the amount of memory and cost per hour (obtained in May 2022) of each instance, and IDs that allows us to identify each one. Message transfer cost in AWS is \$0.09 per GB in the first 10 TB/month and in GCP is \$0.12 per GB in the first 1 TB/month. For storing clients' datasets in AWS and GCP, we respectively chose the Amazon Simple Storage Service (S3)~\cite{aws_s3} in the N. Virginia region (\textit{us-east-1}) and the Cloud Storage~\cite{gcp_storage} in the Iowa region (\textit{us-central1}).
%
\subsection{Training and test times}\label{subsec:expected_exec_time}
%
In order to have the best scheduling map of a Federated Learning application, it is necessary to know clients' and server execution times with corresponding financial costs as well as the communication time between a client and a server, considering all available VMs. However, to run the whole application in order to obtain those execution times and financial costs would be unrealistic.
 
\subsubsection*{Execution times} 

In \cite{malta2019exploring}, Malta~\etal~observed that all training epochs of a centralized Deep Learning training have similar execution times, except for the first one.
Consequently, to obtain the total execution time, only the time of the first two epochs is necessary. The authors proposed then the Equation \ref{eq:malta} that renders $Total\_runtime$, the total time of the application, where $T(Ep_1)$ and $T(Ep_2)$ are the execution times of the first and second training epoch, respectively, and $N_ {ep}$ is the total number of training epochs.

\begin{equation}
\resizebox{0.70\hsize}{!}{$Total\_runtime = T(Ep_1) + (N_{ep} - 1) \times T(Ep_2)$} \label{eq:malta}
\end{equation}

The same behaviour of the previous work was observed in the FL approaches presented in \cite{brum2021wcc} and \cite{brum2021eradrj} where the first FL round has a different execution time from all the other ones, which present similar execution times. Therefore, in this work, to obtain the execution time of our use-case FL application, only its first two rounds were executed. Note that execution time includes both CPU and storage access times. 

Let define the {\em slowdown} $sl\_inst_{jkl}$ as the ratio between the execution time of a dummy application in one of the virtual machines and the execution time in a chosen baseline virtual machine, in our experiments, the AWS instance \textit{g4dn.2xlarge} executing in the N. Virginia region (\textit{us-east-1} region), $vm_{111}$. Thus, the execution time of a round of a client $c_i$ executing on a provider $p_j$, region $r_{jk}$ and virtual machine $vm_{jkl}$ is the sum of training and test steps of client $c_i$ executed on the baseline virtual machine ($train\_bl_{i}$ and $test\_bl_{i}$ respectively) multiplied by the corresponding slowdown ($sl\_inst_{jkl}$), as shown in Equation \ref{eq:t_exec}.
%
\begin{equation}
\resizebox{0.70\hsize}{!}{$t\_exec_{ijkl} = (train\_bl_{i} + test\_bl_{i}) \times sl\_inst_{jkl}$} \label{eq:t_exec}
\end{equation}

Note that once having obtained slowdown values for one dataset size, we can execute the FL application with other dataset sizes, without the need of re-executing the first two rounds of the application in all virtual machine types, except for the baseline. We created a dummy application that simulates the execution of one client in the first two rounds of our use-case FL application to compute this slowdown. Three experiment sets were conducted. 

In the first experiment set, client datasets were stored in AWS and, in each experiment, only one client was executed in a single instance $vm_{jkl}$ of Table \ref{tab:setup} with an attached GPU. The slowdown of a $vm_{jkl}$ is computed by dividing the sum of the second round execution (training and test) times in this instance by the sum of the second round execution in $vm_{111}$, our baseline instance.
Table \ref{tab:exec_times_aws} presents the average values of each step (training and test) of the first (1º r.) and second (2º r.) round, and the computed slowdown (Sl). We executed the client in each instance type three times and observed an average standard deviation of 10.96\%. The second experiment set is similar to the previous one, but client datasets are stored in GCP. Results are presented in Table \ref{tab:exec_times_gcp} with average standard deviation of 11.93\%. Finally, the aggregation task of the server was executed in all virtual machines of AWS and GCP, taking around 0.3 seconds in AWS and 0.2 seconds in GCP.
%
\begin{table}
\caption{Execution times of one client with five local epochs, run in different instances of AWS and GCP and dataset stored in Amazon S3 in N. Virginia region (\textit{us-east-1})} \label{tab:exec_times_aws}
\scriptsize
\begin{center}
\begin{tabular}{|c|c|l|r|r|r|r|c|}
\hline
\multirow{2}{*}{Prov.} & \multirow{2}{*}{Region} & \multirow{2}{*}{VM ID} & \multicolumn{2}{c|}{Training time} & \multicolumn{2}{c|}{Test time} & \multirow{2}{*}{Sl} \\
\cline{4-7}
 & & & 1º r. & 2º r. & 1º r. & 2º r. & \\
\hline
\multirow{4}{*}{AWS} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}N. Virginia\\(\textit{us-east-1})\end{tabular}} & $vm_{111}$ & 04:17 & 06:53 & 03:13 & 03:03 & 1.00 \\
\cline{3-8}
 & & $vm_{112}$ & 08:14 & 31:23 & 16:29 & 19:09 & 5.09 \\
\cline{2-8}
 & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Oregon\\(\textit{us-west-2})\end{tabular}} & $vm_{121}$ & 04:34 & 06:34 & 02:40 & 03:14 & 0.99 \\
\cline{3-8}
 & & $vm_{122}$ & 07:34 & 27:47 & 14:48 & 16:19 & 4.44 \\
\hline
\multirow{5}{*}{GCP} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Iowa\\(\textit{us-central1})\end{tabular}} & $vm_{211}$ & 03:24 & 07:09 & 03:01 & 03:04 & 1.03 \\
\cline{3-8}
 & & $vm_{212}$ & 04:27 & 07:53 & 03:41 & 04:47 & 1.28 \\
\cline{3-8}
 & & $vm_{213}$ & 02:59 & 07:20 & 03:20 & 02:56 & 1.04 \\
\cline{2-8}
 & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Oregon\\(\textit{us-west1})\end{tabular}} & $vm_{221}$ & 03:51 & 07:24 & 02:40 & 03:11 & 1.07 \\
\cline{3-8}
 & & $vm_{222}$ & 03:11 & 07:23 & 03:12 & 03:31 & 1.10 \\
\hline
\end{tabular}
\end{center}
\end{table}
%
\begin{table}
\caption{Execution times of one client with five local epochs, run in different instances of AWS and GCP and dataset stored in GCP Cloud Storage in Iowa region (\textit{us-central1})} \label{tab:exec_times_gcp}
\scriptsize
\begin{center}
\begin{tabular}{|c|c|l|r|r|r|r|c|}
\hline
\multirow{2}{*}{Prov.} & \multirow{2}{*}{Region} & \multirow{2}{*}{VM ID} & \multicolumn{2}{c|}{Training time} & \multicolumn{2}{c|}{Test time} & \multirow{2}{*}{Sl} \\
\cline{4-7}
 & & & 1º r. & 2º r. & 1º r. & 2º r. & \\
\hline
\multirow{4}{*}{AWS} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}N. Virginia\\(\textit{us-east-1})\end{tabular}} & $vm_{111}$ & 04:21 & 03:04 & 00:54 & 00:49 & 1.00 \\
\cline{3-8}
 & & $vm_{112}$ & 06:09 & 04:45 & 01:06 & 01:09 & 1.52 \\
\cline{2-8}
 & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Oregon\\(\textit{us-west-2})\end{tabular}} & $vm_{121}$ & 05:20 & 04:01 & 01:15 & 01:15 & 1.36 \\
\cline{3-8}
 & & $vm_{122}$ & 07:27 & 05:48 & 01:42 & 01:40 & 1.92 \\
\hline
\multirow{5}{*}{GCP} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Iowa\\(\textit{us-central1})\end{tabular}} & $vm_{211}$ & 03:05 & 02:44 & 00:48 & 00:32 & 0.84 \\
\cline{3-8}
 & & $vm_{212}$ & 03:39 & 02:57 & 00:41 & 00:30 & 0.89 \\
\cline{3-8}
 & & $vm_{213}$ & 01:36 & 01:11 & 00:36 & 00:26 & 0.42 \\
\cline{2-8}
 & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Oregon\\(\textit{us-west1})\end{tabular}} & $vm_{221}$ & 04:05 & 02:56 & 00:58 & 00:53 & 0.99 \\
\cline{3-8}
 & & $vm_{222}$ & 02:41 & 02:41 & 01:08 & 00:49 & 0.90 \\
\hline
\end{tabular}
\end{center}
\end{table}

\subsubsection*{Communication times}

Let define $sl\_comm_{xy}$, the communication slowdown of the pair of regions $r_{x}$ (with $x = jk$) and $r_{y}$ (with $y = lm$), as the ratio between the communication time of FL messages between these regions and the communication time in a baseline pair of regions. Here, we define the baseline pair by considering the same region in both sides, the N. Virginia region of AWS (\textit{us-east-1} region). The communication time between regions $r_{x}$ and $r_{y}$ is thus given by Equation \ref{eq:t_comm}, with $train\_comm\_bl$, the communication time of the training messages, and $test\_comm\_bl$, the communication time of the test messages in the baseline pair of regions.

\begin{equation}
\resizebox{0.89\hsize}{!}{$t\_comm_{xy} = (train\_comm\_bl + test\_comm\_bl) \times sl\_comm_{xy}$} \label{eq:t_comm}
\end{equation}

This slowdown $sl\_comm_{xy}$ is computed as the sum of both communication times between client and server divided by the sum of both times in the baseline pair of regions. In order to obtain this communication slowdown, we considered a dummy application with a single client and the server and measured the total time taken by the client to send and receive messages from the server. Neither the server nor the client does any computation with the messages, they only receive them and send them back. Messages had 25,000,000 floating points (size of the dummy model) which correspond to messages of 1GB size. We collected communication slowdown times of 10 executions per pair of regions $r_{jk}$ and $r_{lm}$, having 5 of them with the client in the region $r_{jk}$ and the server in the region $r_{lm}$ and 5 the other way round. Table \ref{tab:comm_times} presents the average times in seconds in all possible pairs of regions and the computed slowdown (Sl). Most standard deviations were below 15\%, with only three above. 

The training communication time is the time taken by the server to send the message $s\_msg_{train}$ with the dummy model (message size of 1GB) and receive back the same model, $c\_msg_{train}$, (message size of 1GB). The test communication time is the time taken by the server to send the message $s\_msg_{aggreg}$ with the model (message size of 1GB) and receive back 10 float points, message $c\_msg_{test}$, representing the possible ML metrics that clients compute (translated to 1.8KB). See Figure \ref{fig:fl_round}. 
%
\begin{table}
\caption{Communication times between each pair of regions. The training phase exchanges a total of 2GB in messages and the test phase exchanges a little more than 1GB in total} \label{tab:comm_times}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Pair of regions} & \multicolumn{2}{c|}{Comm. times (s)} & \multirow{2}{*}{Sl} \\
\cline{2-3} 
 & Training & Test & \\
\hline
\textit{us-east-1} (AWS) \& \textit{us-east-1} (AWS) & 6.68 & 3.59 & 1.00 \\
\hline
\textit{us-east-1} (AWS) \& \textit{us-west-2} (AWS) & 39.67 & 20.30 & 5.84 \\
\hline
\textit{us-east-1} (AWS) \& \textit{us-central1} (GCP) & 22.83 & 12.07 & 3.40 \\
\hline
\textit{us-east-1} (AWS) \& \textit{us-west1} (GCP) & 33.02 & 16.10 & 4.78 \\
\hline
\textit{us-west-2} (AWS) \& \textit{us-west-2} (AWS) & 6.56 & 3.41 & 0.97 \\
\hline
\textit{us-west-2} (AWS) \& \textit{us-central1} (GCP) & 33.25 & 14.53 & 4.65 \\
\hline
\textit{us-west-2} (AWS) \& \textit{us-west1} (GCP) & 20.42 & 10.83 & 3.04 \\
\hline
\textit{us-central1} (GCP) \& \textit{us-central1} (GCP) & 2.30 & 1.21 & 0.34 \\
\hline
\textit{us-central1} (GCP) \& \textit{us-west1} (GCP) & 7.35 & 3.86 & 1.09 \\
\hline
\textit{us-west1} (GCP) \& \textit{us-west1} (GCP) & 4.09 & 2.30 & 0.62 \\
\hline
\end{tabular}
\end{center}
\end{table}
%
\subsection{Analysis of the Scalability of the Proposed Mathematical Formulation}
%
We used \emph{Gurobi Optimizer} \cite{gurobi2022}, a state-of-the-art solver for mathematical programming models, for solving the proposed formulation. In order to analyze its scalability, the number of clients varied from 2 to 50. Furthermore, aiming at increasing the search space, for each VM of Table \ref{tab:setup}, we have created five synthetic VMs. %increasing or reducing the expected execution time and the VM's cost.
Thus, we have a total of 78 VMs, 54 with GPUs and 24 without any GPU.

For the sake of making the problem solution feasible, we set the GPUs and vCPUs limits of all regions and all providers to the infinite constant of Python's math library. We also considered a deadline and a budget of 10,000 seconds and \$30000 per FL round respectively. Figure \ref{fig:scalability_test_big} presents the relation between the number of clients and Gurobi's execution time.
% 
\begin{figure}[htbp]
 \centering
 \includegraphics[width=0.86\columnwidth]{images/scalability_tests_big_deadline_and_budget.pdf}
 \caption{Relation between number of clients and Gurobi's execution time.}
 \label{fig:scalability_test_big}
\end{figure}

We observe in Figure \ref{fig:scalability_test_big} that our mathematical formulation is robust and present the optimal solution, in a realistic time, with a large search space and a considerable number of clients.
%
\begin{table*}
\caption{Theoretical results of a single FL round and 50 clients} \label{tab:theoretical_results_50_clients}
\scriptsize
\begin{center}
\begin{tabular}{|l|l|r|r|l|r|r|r|r|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Scenario}} & \multicolumn{3}{c|}{Optimal selection (model)} & \multicolumn{3}{c|}{User random selection} & \multicolumn{2}{c|}{Difference (\%)} \\ 
\cline{2-9} 
 & \multicolumn{1}{c|}{Setup} & \multicolumn{1}{c|}{Exec. time} & \multicolumn{1}{c|}{Costs (\$)} & \multicolumn{1}{c|}{Setup} & \multicolumn{1}{c|}{Exec. time} & \multicolumn{1}{c|}{Costs (\$)} & \multicolumn{1}{c|}{Exec. time} & \multicolumn{1}{c|}{Costs} \\ 
\hline
GCP(50) &\begin{tabular}[c]{@{}l@{}}clients in $vm_{213}$\\server in $vm_{214}$\end{tabular} & 0:01:45 & 13.84 & \begin{tabular}[c]{@{}l@{}}clients in $vm_{222}$\\server in $vm_{223}$\end{tabular} & 0:03:47 & 18.69 & 53.70 & 25.92 \\ 
\hline
GCP(25)-AWS(25) & \begin{tabular}[c]{@{}l@{}}clients in $vm_{121}$\\server in $vm_{123}$\end{tabular} & 0:10:16 & 13.72 & \begin{tabular}[c]{@{}l@{}}half clients in $vm_{111}$\\and half in $vm_{213}$,\\server in $vm_{214}$\end{tabular} & 0:11:29 & 26.56 & 10.47 & 48.34 \\ 
\hline
\end{tabular}
\end{center}
\end{table*}
%
\subsection{Theoretical Analysis of the Scheduling Results against User Random Selection}
%
In this section, we theoretically analyze the optimal setup results obtained with our model, comparing them with user random selection approaches. In order to obtain a solution that offers a balance between the execution time and financial cost, we set $\alpha = 0.5$. 

Let's consider 50 homogeneous clients with 948 training samples and 522 test samples. As all clients datasets have the same size, we considered the same execution time as the baseline execution time for all the 50 clients. Therefore, for those clients that access their dataset in AWS (resp., GCP), the baseline training time ($train\_bl_{i}$) is 412.94 (resp., 183.53) seconds, and the baseline test time ($test\_bl_{i}$) is 182.77 (resp., 49.47) seconds. Regarding communication, messages of the server as well as the training message of clients have 0.54GB of size and the test message from clients has 1.81KB of size. The total value for the communication baseline time ($train\_comm\_bl + test\_comm\_bl$) is 27.26 seconds.

We consider two data placement scenarios: {\em GCP(50)} where all datasets are stored in GCP Cloud Storage and {\em GCP(25)-AWS(25)} where datasets of 25 clients are stored in GCP Cloud Storage and the other 25 in AWS S3. For each scenario, the respective optimal setup results of our model are compared to a given user selection approach, also described in the following. Note that all values are computed from the slowdowns presented in the previous sections.

\subsubsection*{- GCP(50) scenario} 
%
Our model proposes a optimal setup where the 50 clients and the server should be in the Iowa region of GCP (\textit{us-central1} region), with all clients in different \textit{n1-standard-8} VMs with a Volta GPU in each ($vm_{213}$) and the server in a \textit{e2-standard-4} VM ($vm_{214}$). The $vm_{213}$ is the most expensive VM in GCP but has the smallest execution time. On the other hand, we considered a random approach where all clients and the server are placed in the Oregon region of GCP (\textit{us-west1} region), using the same VM types, assigning $vm_{222}$ to clients and $vm_{223}$ to the server. Compared to this approach, the optimal one reduces in 53.70\% the execution time and in 25.92\% the costs.

\subsubsection*{- GCP(25)-AWS(25) scenario} 
%
Instead of placing the clients near the datasets in each cloud provider, our mathematical model proposes to place all the 50 clients and the server in the Oregon region of AWS (\textit{us-west-2}): each client in different \textit{g4dn.2xlarge} VM ($vm_{121}$), which is the fastest VM in all regions of AWS, and the server in a \textit{t2.xlarge} VM ($vm_{123}$). On the other hand, we consider a random approach where all clients are placed near the datasets in the fastest VMs of the chosen region and the server in one of the cheapest VMs. Thus, for such a configuration, we used the \textit{g4dn.2xlarge} VM in the N. Virginia region ($vm_{111}$) for the 25 clients with dataset in AWS, the \textit{n1-standard-8} VM with a Volta GPU in the Iowa region ($vm_{213}$) for the ones with dataset in GCP, and the \textit{e-standard-4} VM in the Iowa region ($vm_{214}$) to the server. In this case, the FL round in the optimal setup reduces in 10.47\% the execution time and in 48.34\% the costs.

Table \ref{tab:theoretical_results_50_clients} summarizes these two scenarios. It presents the location of the datasets (Scenario), the optimal setup, the execution time and costs computed by the mathematical formulation, along with the random approaches described above, and the difference between the latter and the optimal setup. This difference is computed by $\frac{v_r-v_o}{v_r}$, where $v_r$ is the random approach value and $v_o$ is the optimal one.

%
\subsection{Analysis of the Scheduling Results in a Multi-cloud Platform}
%
For each of the current experiments, we have had to respect the maximum number of global and per region vCPUs and GPUs that a user can allocate in each cloud provider. In GCP, vCPUs (both global and per region one) and GPUs are respectively limited to 40 and 4. In AWS, the limit of the N. Virginia (\textit{us-east-1}) region vCPUs is 52 and of the Oregon region (\textit{us-west-2}) is 36. On the other hand, there is no restriction for the number of global vCPU and the GPU limit is included in the vCPU one. Thus, we have kept the infinity constant for these limits in AWS. We use the same input data (baseline execution and communication time) as the previous experiment for all clients $c \in C$.

We have reproduced the best FL scenario presented in \cite{brum2021eradrj} which consists of four clients with equally divided datasets, that execute 10 FL rounds with 5 local epochs each. Each client has 948 training samples and 522 test samples, with 10\% of TIL-positive in each dataset. We have then considered three possible dataset placement scenarios: AWS(4), GCP(4) and AWS(2)-GCP(2). In AWS(4), all datasets are stored in AWS, while in GCP(4) they are placed in GCP. In the last scenario, AWS(2)-GCP(2), half of the datasets is stored in AWS, while the other half is stored in GCP.

Our model uses only three different VMs to place the clients in each of the above three scenarios. For sake of evaluation comparison, for each scenario, we also created two user random selection assignments. In the case of AWS(4) (resp., GCP(4)) scenarios, the first assignment allocates clients and the server in the cheapest VMs (with GPU, in case of clients) within the same cloud region in AWS (resp., GCP) where is located the dataset of the corresponding client, while the second assignment has a similar allocation but on the other cloud provider, i.e., GCP (resp., AWS). 
For the GCP(2)-AWS(2) scenario, the two user selection assignments consider that clients are allocated in cheapest VMs with GPU in the same region of their datasets but the server changes position, being in AWS in the first setup and in GCP in the second. All the scheduling assignments are described in Table \ref{tab:vms_setup}, and the configuration of each VM can be found in Table \ref{tab:setup}.
%
\begin{table*}
\caption{VMs setup for optimal and random scheduling schemes for all scenarios with 4 clients} \label{tab:vms_setup}
\scriptsize
\begin{center}
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{Scenarios} & Optimal selection (model) & 1$^{st}$ user random selection & 2$^{nd}$ user random selection \\ 
\hline
AWS(4) & \begin{tabular}[c]{@{}l@{}}$c_1$ in $vm_{121}$, $c_2$ in $vm_{121}$,\\$c_3$ in $vm_{121}$, $c_4$ in $vm_{121}$, $s$ in $vm_{123}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$c_1$ in $vm_{111}$, $c_2$ in $vm_{111}$,\\$c_3$ in $vm_{111}$, $c_4$ in $vm_{111}$, $s$ in $vm_{113}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$c_1$ in $vm_{211}$, $c_2$ in $vm_{211}$,\\$c_3$ in $vm_{211}$, $c_4$ in $vm_{211}$, $s$ in $vm_{214}$\end{tabular} \\ 
\hline
GCP(4) & \begin{tabular}[c]{@{}l@{}}$c_1$ in $vm_{213}$, $c_2$ in $vm_{213}$,\\$c_3$ in $vm_{213}$, $c_4$ in $vm_{213}$, $s$ in $vm_{214}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$c_1$ in $vm_{211}$, $c_2$ in $vm_{211}$,\\$c_3$ in $vm_{211}$, $c_4$ in $vm_{211}$, $s$ in $vm_{214}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$c_1$ in $vm_{111}$, $c_2$ in $vm_{111}$,\\$c_3$ in $vm_{111}$, $c_4$ in $vm_{111}$, $s$ in $vm_{113}$\end{tabular} \\
\hline
AWS(2)-GCP(2) & \begin{tabular}[c]{@{}l@{}}$c_1$ in $vm_{121}$, $c_2$ in $vm_{121}$,\\$c_3$ in $vm_{121}$, $c_4$ in $vm_{111}$, $s$ in $vm_{123}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$c_1$ in $vm_{111}$, $c_2$ in $vm_{111}$,\\$c_3$ in $vm_{211}$, $c_4$ in $vm_{211}$, $s$ in $vm_{113}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}$c_1$ in $vm_{111}$, $c_2$ in $vm_{111}$,\\$c_3$ in $vm_{211}$, $c_4$ in $vm_{211}$, $s$ in $vm_{214}$\end{tabular} \\
\hline
\end{tabular}
\end{center}
\end{table*}

We first present the execution time and the cost for a single round of FL to all setups in Table \ref{tab:theoretical_results}. The optimal values come from the mathematical formulation and the random scheduling setups are computed using the slowdowns from the previous subsections. We also present how much the optimal setup gains in terms of percentage from the random scheduling schemes, computed by $\frac{v_r-v_o}{v_r}$, where $v_r$ is the user random selection approach value and $v_o$ is the optimal one. Note that a negative percentage value means that the optimal value is bigger than the random one.
%
\begin{table*}
\caption{Theoretical results with single FL round} \label{tab:theoretical_results}
\scriptsize
\begin{center}
\begin{tabular}{|l|r|r|l|r|r|r|r|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Scenarios}} & \multicolumn{2}{c|}{Optimal selection (model)} & \multicolumn{3}{c|}{User random selection} & \multicolumn{2}{c|}{Difference (\%)} \\ 
\cline{2-8} 
 & \multicolumn{1}{c|}{Exec. time} & \multicolumn{1}{c|}{Costs (\$)} & \multicolumn{1}{c|}{\#} & \multicolumn{1}{c|}{Exec. time} & \multicolumn{1}{c|}{Costs (\$)} & \multicolumn{1}{c|}{Exec. time} & \multicolumn{1}{c|}{Costs} \\ 
\hline
\multirow{2}{*}{AWS(4)} & \multirow{2}{*}{0:10:16} & \multirow{2}{*}{1.13} & 1$^{st}$ & 0:10:23 & 1.13 & 1.09 & 0.53 \\ 
\cline{4-8} 
 & & & 2$^{nd}$ & 0:10:23 & 1.30 & 1.05 & 13.44 \\ 
\hline
\multirow{2}{*}{GCP(4)} & \multirow{2}{*}{0:01:47} & \multirow{2}{*}{1.12} & 1$^{st}$ & 0:03:25 & 0.95 & 47.69 & -18.05 \\
\cline{4-8} 
 & & & 2$^{nd}$ & 0:04:21 & 0.81 & 58.81 & -37.88 \\
\hline
\multirow{2}{*}{AWS(2)-GCP(2)} & \multirow{2}{*}{0:10:16} & \multirow{2}{*}{1.13} & 1$^{st}$ & 0:10:23 & 1.16 & 1.09 & 2.64 \\
\cline{4-8} 
 & & & 2$^{nd}$ & 0:11:29 & 1.33 & 10.47 & 15.51 \\
\hline
\end{tabular}
\end{center}
\end{table*}

We can observe from Table \ref{tab:theoretical_results} that our mathematical model presents better results in all scenarios with an average execution time reduction of 20.03\% compared to the randomly selected scenarios. Regarding the monetary costs, the average difference is -3.97\%. This negative difference comes from scenario GCP(4), where the optimal setup is more expensive than both random scenarios (by 18.05\% and 37.88\%), but with a higher reduction in the execution time (47.69\% and 58.81\%).

The above comparisons show that placing the clients (and server) as close as possible to the dataset does not always provide the best execution time. For example, in the scenario AWS(4), where all datasets are in the N. Virginia region of AWS and our mathematical formulation places clients and the server in the Oregon region of AWS, the single FL round has presented a small reduction in both execution time and total costs when compared to the first user selection approach, where all allocated VMs are in the N. Virginia region. We should point out that a FL application usually executes for several rounds, which increases the absolute difference in time and costs between the optimal setup and the random ones. 

Results from scenario AWS(2)-GCP(2) show that the misplacement of the server can increase both execution time and costs. Although the execution time of all clients is the same in both random setups, the communication time between the slowest client and the server varies. The clients whose datasets are in AWS take longer to execute than the other two, and communication time inside the same AWS region is much lower than between both providers. Moreover, the transfer costs change according to the server placement. If it is on AWS, the cost is less (\$0.09 per GB) than when it is in GCP (\$0.12 per GB). Therefore, the difference in execution time and costs between the two random setups for this scenario can be explained.

Finally, we did a real deployment and executed all setups in both cloud providers (AWS and GCP) with 10 FL epochs. Table \ref{tab:optimization_of_runtime_costs} summarizes the obtained results, showing that the optimal solution allows an average execution time reduction of 21.07\%, with an average cost increase of only 4.30\%. 
%
\begin{table*}
\caption{Real Cloud execution with 10 FL rounds} \label{tab:optimization_of_runtime_costs}
\scriptsize
\begin{center}
\begin{tabular}{|l|r|r|l|r|r|r|r|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Scenarios}} & \multicolumn{2}{c|}{Optimal selection (model)} & \multicolumn{3}{c|}{User random selection} & \multicolumn{2}{c|}{Difference (\%)} \\ 
\cline{2-8} 
 & \multicolumn{1}{c|}{Exec. time} & \multicolumn{1}{c|}{Costs (\$)} & \multicolumn{1}{c|}{\#} & \multicolumn{1}{c|}{Exec. time} & \multicolumn{1}{c|}{Costs (\$)} & \multicolumn{1}{c|}{Exec. time} & \multicolumn{1}{c|}{Costs} \\
\hline
\multirow{2}{*}{AWS(4)} & \multirow{2}{*}{1:31:18} & \multirow{2}{*}{10.66} & 1$^{st}$ & 1:35:14 & 10.87 & 4.12 & 1.92 \\ 
\cline{4-8} 
 & & & 2$^{nd}$ & 1:55:03 & 13.59 & 20.64 & 21.56 \\ 
\hline
\multirow{2}{*}{GCP(4)} & \multirow{2}{*}{0:22:00} & \multirow{2}{*}{11.98} & 1$^{st}$ & 0:36:54 & 9.61 & 40.38 & -24.61 \\
\cline{4-8} 
 & & & 2$^{nd}$ & 0:51:22 & 8.53 & 57.18 & -40.34 \\
\hline
\multirow{2}{*}{AWS(2)-GCP(2)} & \multirow{2}{*}{1:36:09} & \multirow{2}{*}{10.92} & 1$^{st}$ & 1:37:37 & 11.25 & 1.51 & 2.93 \\
\cline{4-8} 
 & & & 2$^{nd}$ & 1:38:42 & 12.51 & 2.59 & 12.71 \\
\hline
\end{tabular}
\end{center}
\end{table*}

We can observe in the table that the computed differences between the optimal values and the random ones are close to the theoretical results (Table \ref{tab:theoretical_results}) but not equal. Besides, the real cloud differences in the second random setup of scenario AWS(4) are far from the theoretical ones. In~\cite{leitner2016patterns}, Leitner \etal~have extensively evaluated the performance of different cloud platforms, showing that the performance of IO-bound applications in AWS varies a lot even in the same VM. Hence, since our application transfers data from memory to the GPU at least two times per round, the variation of IO performance has a negative impact on execution times, which explains the difference found between Table \ref{tab:theoretical_results} and Table \ref{tab:optimization_of_runtime_costs}.

\subsection{Discussion about the multi-cloud environment and results} \label{subsec:discussion}
%
Firstly, concerning the AWS-GCP environment of our experiments, all AWS EC2 instances were almost always available for deployment, although, they frequently presented performance variation. Particularly, the Volta GPU instance had poor unexpected performance, which led us to remove it from the model's search space. On the contrary, GCP instances presented a stable performance. We also observed that the time taken to access datasets allocated in AWS S3 (Table \ref{tab:exec_times_aws}) was higher than the time to access the corresponding datasets in the GCP Cloud Storage (Table \ref{tab:exec_times_gcp}). Such behavior is coherent with other ones from the related literature. In~\cite{leitner2016patterns} Leitner \etal~present extensive experiments regarding the performance and predictability of different VM instance types in many cloud providers. The authors concluded that, in general, AWS has worse performance and is more unpredictable than GCP.

We also observe that the $\alpha$ parameter of our model has a low impact. The results with $\alpha$ equal to 0.5, 0, or 1 produced the same execution times and costs, for most of the experiments.

Our theoretical analysis shows that the execution time given by the proposed model is reduced by up to 58.81\% when compared to random scenarios with four FL clients in the cloud whose datasets are stored in GCP (scenario GCP(4)). Considering 50 clients, with half of them storing their dataset in AWS and the other half in GCP (scenario AWS(25)-GCP(25)), the monetary costs and execution time are reduced by up to 48.34\% and 10.47\% respectively.

In the experiments conducted in the AWS-GCP platform, scenario GCP(4) yielded a reduction of 40.38\% on the execution time when placing clients in the same region of the dataset in the most expensive VM type with a monetary cost increase of 24.61\%. 

When comparing, for a single FL application round, the theoretical execution times and the ones obtained in the AWS-GCP platform, we observe a difference of 11.14\% in scenario AWS(4), -22.96\% in scenario GCP(4), and 6.42\% in scenario AWS(2)-GCP(2). Although in scenario GCP(4), such a difference in percentage is higher than the other two, the absolute value is smaller: only 25 seconds of difference compared to 1 minute and 10 seconds in AWS(4) and 40 seconds in AWS(2)-GCP(2). Moreover, Ward and Barker~\cite{Ward2014} have shown in 2014 that the same VM type could vary its performance by up to 29\%. The authors associated this variation with the oversold physical machine underneath the VMs and other multi-tenanted phenomena. In our experiments, we observe that the variation among the same VM type is smaller nowadays, but still present.

\section {Conclusion and Future Work} \label{sec:conclusions}
%
This paper has presented a mathematical formulation for a Cross-Silo Federated Learning task scheduling problem in a multi-cloud scenario, aiming at minimizing its execution time and monetary cost. This formulation is part of a framework proposal to execute Federated Learning applications in a multi-cloud scenario. Theoretical results show that the proposed model is robust and scales with the growth of the number of clients and available virtual machines. 

Furthermore, in a real scenario using  Amazon-GCP multi-cloud platform with 4 clients and datasets stored in AWS S3 and GCP Cloud Storage, the optimal setup offered an improvement by up to 57.18\% in the execution time and up to 21.56\% in the monetary costs when compared to random selection approach.

In future work, we aim introducing heterogeneity in clients' datasets and models, to evaluate the proposed approach in terms of performance and  quality results. Besides, we intend to use  Spot instances, which are offered with a huge discount by cloud providers, but can be revoked. In this case, upon the revocation, our framework will need to to reschedule the interrupted tasks dynamically through a dynamic scheduler module. Moreover, we are currently working on a fault-tolerant module in our framework not to loose all computation when a revocation occurs.

\section*{Acknowledgment}

This research is supported by \textit{Programa Institucional de Internacionaliza\c{c}\~{a}o} (PrInt) from CAPES (process number 88887.310261/2018-00), by CNPq (process number 145088/2019-7), by the \textit{Coordena\c{c}\~{a}o de Aperfei\c{c}oamento de Pessoal de N\'{i}vel Superior} (CAPES - Finance Code 001), by Project Universal/CNPq n$^o$ 404087/2021-3 and CNE/FAPERJ n$^o$ E-26/201.012/2022(271103).

==> old_articles/wcc_text.tex <==
\begin{abstract}
This paper proposes Multi-FedLS, a Cross-silo Federated Learning (FL) framework for a multi-cloud environment aiming at minimizing financial cost as well as execution time. It comprises four modules: Pre-Scheduling, Initial Mapping, Fault Tolerance, and Dynamic Scheduler. Given an application and a multi-cloud environment, the Pre-Scheduling module runs experiments to obtain the expected execution times of the FL tasks and communication delays. The Initial Mapping module receives these computed values and provides a scheduling map for the server and clients' VMs. Finally, Multi-FedLS deploys the selected VMs, starts the FL application, and monitors it. The Fault Tolerance (FT) module includes fault tolerance strategies in the FL application, such as checkpoint and replication, and detects some anomalous behaviors. In case of an unexpected increase in the communication delay or a VM failure, the FT module triggers the Dynamic Scheduler Module in order to select a new VM and resume the concerned tasks of the FL application. Some preliminary experiments are presented, confirming that some proposed strategies are crucial to efficiently execute an FL application on a multi-cloud environment.

\end{abstract}

\begin{IEEEkeywords}
Federated Learning Framework, Multi-Cloud Environment, Efficient Resource Allocation
\end{IEEEkeywords}

\section{Introduction}

Federated Learning (FL) is a recent type of distributed Machine Learning (ML) in which the participating clients do not share their private data~\cite{shen2021difference_distributed_federated_learning}. The clients federation solves the learning task by having a coordinated central server that keeps the current global model. Each client trains its local model on its local data set and communicates only the model weights to the server, updating then the global model.

The server-clients architecture of FL, also called Model-Centric Federated Learning~\cite{yang2019federated}, is classified into Cross-Device or Cross-Silo Federated Learning, depending on the client's type. In Cross-Device Federated Learning, clients are low-powered devices, like mobile phones~\cite{mcmahan2017communication} or IoT devices~\cite{nguyen2021iot} while in Cross-Silo Federated Learning, clients are companies or institutions (\eg, hospitals~\cite{rajendran2021cloud}) with similar datasets willing to create a central model. In this second type of FL, the central server can assume that all clients are available during the whole execution, as they are powerful machines or even clusters.

Nowadays, training ML algorithms uses a huge amount of generated data. Data are often stored using cloud storage services \cite{li2010cloudcmp} whose performance can vary. Besides the latter, cloud providers also offer Virtual Machines (VMs) with different accelerators in a service generically called Infrastructure-as-a-Service (IaaS). For example, the Amazon Web Services (AWS) offers GPUs attached to pre-defined VMs types, whose architectures vary from Kepler to Ampere~\cite{aws_gpu_instances}, while Google Cloud Platform (GCP) allows the user to attach GPUs or TPUs to a pre-defined or custom instance type~\cite{gcp_gpus, gcp_tpus}.

Thus, in a multi-cloud environment, an FL framework should choose the cloud provider, VM types and regions, and the minimum required network bandwidth for each client and server. A wrong choice can result in a considerable increase in the execution cost of an FL application~\cite{ostermann2010performance, kotas2018comparison}. In other words, the allocation of cloud resources is critical for an efficient execution of FL applications in clouds. Therefore, a multi-cloud environment should cope with the problem of configuring the clouds, FL execution monitoring, and selection of a new VM whenever one of the current allocated ones becomes unavailable. 

Although there is a vast literature on scheduling and resource management of FL jobs~\cite{yang2020scheduling, xia2020multi_armed_scheduling, ren2021joint_resource_allocation, buyukates2021timely_communication, pilla2021optimal}, most of them focus on Cross-Device Federated Learning scenarios, where low-powered resources frequently become offline during the training process. The scheduling and resource provisioning problems of Cross-Silo FL applications can be related to the scheduling of distributed Machine Learning (ML) applications~\cite{mohamadi2019distributed_ml_stragglers, liu2020distributed_ml_networks, yu2021distributed_ml_locality} as there is the assumption that the workers are always available. However, there are two main differences between scheduling distributed ML and FL: (i) in ML, the scheduler assumes that all workers have the same amount of data, and (ii) data can be shared among workers. 

In this work, we propose Multi-FedLS, an architecture of a Cross-silo FL framework. The framework comprises four modules: Pre-Scheduling, Initial Mapping, Fault Tolerance, and Dynamic Scheduler. The first module collects information about the FL application and the cloud environment when there is no previous knowledge about them, such as the expected execution time of the FL tasks and communication delays. Then, the Initial Mapping receives these computed values and provides, through a mathematical formulation, a scheduling map of the server and clients, aiming at minimizing financial costs and execution times. Finally, Multi-FedLS deploys the selected VMs, starts the FL application, and monitors it. The Fault Tolerance module is responsible for including fault tolerance strategies in the FL application, such as checkpoint and replication. In case of an unexpected increase in the communication delay or a VM failure, that module triggers the Dynamic Scheduler Module to select a new VM and resume the concerned tasks of the FL application.

The remaining of this paper is organized as follows. Section~\ref{sec:tools_fl} presents the main available tools for federated learning. The proposed Multi-FedLS framework, introduced in Section~\ref{sec:proposal}, is a Flower-based framework to execute Federated Learning Applications on Multi-clouds. Section~\ref{sec:experiments} describes the Pre-Scheduling components and presents some preliminary experiments. Finally, Section \ref{sec:conclusion}, concludes the paper and present some future research directions.

\section{Available Tools for Federated Learning} \label{sec:tools_fl}

There are several tools for executing Federated Learning applications in the literature. TensorFlow Federated (TFF)~\cite{tensorflowfederated} is a Google's library to execute Federated Learning applications in a simulation environment based on the well-known TensorFlow (TF) API. TFF gives the user two API layers: Federated Learning (TFF-FL) API for executing basic FL algorithms and Federated Core (TFF-FC) API for implementing new FL algorithms. The authors claim that TFF can simulate the FL environment in several machines with multiple GPUs\footnote{https://www.tensorflow.org/federated/tutorials/simulations\_with\_accelerators, last accessed in January 2022}. However, we could not find any explanation on how to set up this multi-machine simulation in TFF tutorials\footnote{https://www.tensorflow.org/federated/tutorials/simulations, last accessed in January 2022}.

PySyft and PyGrid are two components of a tool focused on Data-Centric Federated Learning~\cite{ryffel2018pysyft}, in which users compute data they cannot see. In this type of FL, the actors are Data Scientists, which do not have any data, while the Data Owner holds all data and receives computational requests from the Scientists. 

Burlachenko \etal~proposed FL\_PyTorch, an FL simulation tool built on top of the PyTorch API~\cite{paszke2019pytorch}, which helps researchers to develop new FL aggregation techniques. However, such a tool is focused only on simulation.

Federated AI Technology Enabler (FATE)~\cite{fate} provides a framework to support not only the FL training step, but the whole process: data pre-processing, training, and inference steps. FATE has several modules to handle different features of the environment for: (i) describing FL algorithms, data structures, and communication channels; (ii) post-training inference and managing the whole FL pipeline; and (iii) helping users to explore the trained models through visualization tools. 

Flower \cite{beutel2021flower} is an open-source FL framework that deals with heterogeneous clients in simulated or real-world scenarios, allowing the use of any ML framework underneath it (TensorFlow, PyTorch, or a custom one). Besides, Flower can execute in several environments with different operating systems and hardware settings. Researchers can expand Flower's code in order to implement new FL algorithms. Due to its modular structure, the final user only needs to implement a few functions for transforming a regular ML application into a federated one.

We have adopted Flower in our proposal because of its simple architecture and the possibility of execution in real and heterogeneous environments.

\section{Multi-FedLS: A Framework based on Flower to execute Federated Learning Applications on Multi-clouds}
\label{sec:proposal}

An FL application contains two types of tasks: server and clients. The clients train their local model with their private data while the server coordinates the learning by aggregating the clients' model weights. 
 
A communication round is the processing unit of an FL application and it is composed by five steps: (i) the server sends the initial weights to clients; (ii) the clients train their local model with their training dataset and send the updated weights back to the server; (iii) the server receives all updates, aggregates them and sends back to the clients the new weights; (iv) the latter update their local weights with the received ones, evaluate the model with their test dataset and send the evaluation metrics to the server; and (v) the server receives all evaluation metrics, aggregates them and starts the next communication round. Note that there are two communication barriers in a single round. Thus, due to those synchronization barriers, any increase in the communication time has an impact in the total FL execution time. It is worth remarking that the clients' datasets may be spread in several storage systems of different cloud providers.

The proposed Multi-FedLS framework is composed by four modules: the Pre-scheduling, the Initial Mapping, the Fault Tolerance, and the Dynamic Scheduler modules. 

Figure~\ref{fig:framework_design} shows the proposed architecture for the Multi-FedLS framework. 
%
\begin{figure}[htbp]
 \centering
 \includegraphics[width=0.48\textwidth]{images/framework_design.pdf}
 \caption{Architecture of Multi-FedLS}
 \label{fig:framework_design}
\end{figure}

\subsection{Pre-Scheduling Module} \label{sec:pre_scheduling}

The Multi-FedLS framework requires information from FL applications, the available VMs, and cloud providers to define the best mapping of clients and server to VMs in the multi-cloud environment. Some types of information, such as the number of clients, number of communication rounds, number of training epochs, location of each client's dataset, and VM prices, are easily obtained. On the other hand, many others, such as the communication delay between cloud regions or the execution time of clients in different VMs, require the execution of experiments to be known. We also point out that, due to the communication barriers, any increasing in the communication time has an impact in the total FL execution time. Consequently, it is crucial to evaluate the time spent sending messages between different cloud regions to define the best VMs locations for the clients and server processes in the multi-cloud environment. Also, the execution time of FL clients and server may vary according to the types and regions of the allocated VMs. Hence, such an information is also necessary when selecting the most suitable VMs for the FL application. 

Thus, using dummy applications, the Pre-Scheduling module is responsible for executing some tests for obtaining all the above discussed values. 

\subsection{Initial Mapping}\label{sec:static_scheduler}

Receiving as input (i) the datasets locations, (ii) the machine learning procedures, and (iii) data provided by the Pre-Scheduling module, the Initial Mapping module generates an allocation map of the clients and server for a multi-cloud environment, aiming at minimizing both the total execution time and financial costs of the FL application. The mapping problem can be solved using either a mathematical formula or, in case the execution time is prohibitive, a heuristic.

Public cloud providers offer computing resources through a plethora of Virtual Machine (VM) instances with different capacities. They provide these instances under several contract models that differ according to the availability guarantees and prices. Under the classic {\em On-demand} pricing model, a user pays for VM instances per hour or second without any long-term commitment or upfront payment. In the other hand, many providers also offer their spare unused computing capacity, as {\em Spot VM Instances}, at significant discounts comparing to their standard {\em On-demand} prices. However, such price advantages come with the caveat of having no guarantees of VM availability. In order to reduce costs, Multi-FedLS can use Spot VMs, that, although cheaper than On-demand ones, can be revoked at any time by the cloud provider. Consequently, both a monitoring tool and a dynamic scheduler are necessary to reallocate the clients and server in case of such revocations.

\subsection{Tolerating Faults and Dynamic Scheduler} \label{sec:dynamic_scheduler}

Usually, Federated Learning tools can deal with clients' revocations along the execution. When Flower detects a client failure, the server ignores the faulty client by aggregating only the results from the other ones. Furthermore, it is possible to define a minimum number of available clients to start a new communication round. Since in cross-silo FL there are few clients, and the lost of one of them can compromise the learning outcomes, in our proposal, when a client is revoked, it is re-started from a checkpoint in a new VM, or in some cases, it is replicated to avoid new VM deploying and recovery overheads. The selection of a new VM should consider the characteristics of the used cloud providers. For example, if the Amazon Web Services stores a dataset only in one region, a VM belonging to this region is more suitable for executing the corresponding client than VMs from others regions. 

Most FL tools do not handle faults on the server side. In Flower, when the server of an application fails, all clients finish their executions with an error. Thus, Multi-FedLS needs to handle possible server revocations by implementing fault-tolerant techniques on the server side. Although Flower does not have an automatic way to save the model updates on the server side, after each communication round, it allows the users to modify the server code to implement checkpointing \footnote{https://flower.dev/docs/saving-progress.html}. In this case, Multi-FedLS has to deploy another VM to execute the server, considering all clients' positions, the communication times, and costs.

\section{Pre-Scheduling Components and Preliminary Experiments} \label{sec:experiments}

In this section, we describe in more details the Pre-Scheduling module and introduce some results for a case study application. The module receives input information about the FL application and the environment. Concerning the application, it requires the number of clients, the datasets' location, the number of communication rounds, and the number of epochs trained in each round. Regarding the multi-cloud environment, it needs information about the cloud regions and the possible VMs types that can execute the FL tasks.

The Pre-Scheduling module automatically gets the following data of the multi-cloud environment: (i) regions of each cloud provider, (ii) number of Availability Zones (AZs, described later) at each region, and (iii) characteristics of the offered VMs, \eg vCPUs, memory, GPU type, and GPU memory.
Then, this module executes tests to compute the communication delay among all cloud regions and the expected execution time of each client at every instance type. 

For the experiments, we have chosen a Federated Learning application for a Tumor Infiltrating Lymphocytes (TIL) classifier, described in \cite{brum2021wcc, brum2021eradrj}, and the Amazon Web Services (AWS) and Google Cloud Provider (GCP), as cloud providers.

\subsection{Communication delay between cloud regions} \label{subsec:rtt_cloud_regions}

Cloud providers divide their physical infrastructure into cloud regions, which are independent and isolated geographic areas~\cite{aws_regions_zones, gcp_regions_zones}. Those regions are also divided as isolated failure points, called Availability Zones (AZs), to improve the reliability of each region. If a user deploys VMs in two AZs of the same region and one of them fails, the other one may continue executing. An AZ is one or more data centers inside a building, being a region a collection of AZs inside a small geographical area (usually within one city). In February 2022, GCP had three or four zones at each region, and AWS contained three to six availability zones at each cloud region. Cloud providers identify each AZ by a letter at the end of the region's name, normally one between \textit{a} and \textit{f}.

In our experiments, the Pre-Scheduling module executes a dummy application with one server and single client to measure the message exchange time between them. That application used a floating point vector with the size of the VGG16 CNN model~\cite{vgg_paper}, which has more than 130 millions weights, to represent the FL model. The training message time is the time taken by the server to send the vector and receive it back, while the test message time is the time taken by the server to send the vector and receive a dictionary with 8 dummy keys and values, representing the possible machine learning metrics. In the presented experiments, the following regions and cloud providers were considered: \textit{us-east-1} in AWS and \textit{us-central1} (GCP) in GCP. 

Tables \ref{tab:rpc_times_training} and \ref{tab:rpc_times_test} show the average times of 10 executions of the dummy application in several scenarios. The execution times were obtained in different days and times of the week during a period of one month. 
% 
\begin{table*}[htbp]
\caption{Required times to exchange a training message between Availability Zones of regions \textit{us-east-1} (AWS) and \textit{us-central1} (GCP). Times in seconds} \label{tab:rpc_times_training}
\begin{center}
\scriptsize
\begin{tabular}{cc|cccccr|rrrr|}
\cline{3-12}
 & & \multicolumn{6}{c|}{\begin{tabular}[c]{@{}c@{}}AWS\\ \textit{us-east-1}\end{tabular}} & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}GCP\\ \textit{us-central1}\end{tabular}} \\ \cline{3-12} 
 & & \multicolumn{1}{c|}{\textit{1a}} & \multicolumn{1}{c|}{\textit{1b}} & \multicolumn{1}{c|}{\textit{1c}} & \multicolumn{1}{c|}{\textit{1d}} & \multicolumn{1}{c|}{\textit{1e}} & \multicolumn{1}{c|}{\textit{1f}} & \multicolumn{1}{c|}{\textit{1-a}} & \multicolumn{1}{c|}{\textit{1-b}} & \multicolumn{1}{c|}{\textit{1-c}} & \multicolumn{1}{c|}{\textit{1-f}} \\ \hline
\multicolumn{1}{|c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}AWS\end{tabular}}} & \textit{1a} & \multicolumn{1}{c|}{29.74±1.13} & \multicolumn{1}{c|}{31.31±0.71} & \multicolumn{1}{r|}{30.71±1.70} & \multicolumn{1}{r|}{32.49±2.05} & \multicolumn{1}{r|}{29.55±1.03} & 30.84±0.84 & \multicolumn{1}{r|}{115.24±58.23} & \multicolumn{1}{r|}{94.28±45.02} & \multicolumn{1}{r|}{119.21±47.17} & 104.24±45.71 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1b} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{30.15±0.80} & \multicolumn{1}{r|}{30.46±0.69} & \multicolumn{1}{r|}{30.79±1.51} & \multicolumn{1}{r|}{31.66±1.33} & 29.97±0.52 & \multicolumn{1}{r|}{157.29±25.51} & \multicolumn{1}{r|}{149.25±13.75} & \multicolumn{1}{r|}{159.66±20.19} & 140.89±15.71 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1d} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{30.77±1.41} & \multicolumn{1}{r|}{31.03±3.61} & \multicolumn{1}{r|}{32.28±2.24} & 30.59±1.4 & \multicolumn{1}{r|}{168.23±22.12} & \multicolumn{1}{r|}{164.59±16.08} & \multicolumn{1}{r|}{171.67±12.92} & 165.71±20.05 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1c} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{r|}{-} & \multicolumn{1}{r|}{30.96±1.89} & \multicolumn{1}{r|}{31.89±2.27} & 31.89±3.65 & \multicolumn{1}{r|}{157.13±18.15} & \multicolumn{1}{r|}{151.04±16.51} & \multicolumn{1}{r|}{147.93±15.03} & 151.06±16.90 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1e} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{r|}{29.38±1.18} & 29.45±0.95 & \multicolumn{1}{r|}{148.45±16.40} & \multicolumn{1}{r|}{139.53±17.77} & \multicolumn{1}{r|}{136.25±19.22} & 137.37±19.16 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1f} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & 29.46±0.42 & \multicolumn{1}{r|}{161.93±17.63} & \multicolumn{1}{r|}{148.60±9.63} & \multicolumn{1}{r|}{150.48±20.28} & 147.79±11.05 \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}GCP\end{tabular}}} & \textit{1-a} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{r|}{12.58±2.19} & \multicolumn{1}{r|}{16.80±3.21} & \multicolumn{1}{r|}{11.76±2.03} & 15.26±2.80 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1-b} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{r|}{20.49±1.54} & \multicolumn{1}{r|}{17.61±2.79} & 17.59±2.02 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1-c} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{r|}{13.37±2.48} & 17.80±2.69 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1-f} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & 19.97±0.94 \\ \hline
\end{tabular}
\end{center}
\end{table*}
%
\begin{table*}[htbp]
\caption{Required times to exchange a test message between Availability Zones of regions \textit{us-east-1} (AWS) and \textit{us-central1} (GCP). Times in seconds} \label{tab:rpc_times_test}
\begin{center}
\scriptsize
\begin{tabular}{cc|cccccr|rrrr|}
\cline{3-12}
 & & \multicolumn{6}{c|}{\begin{tabular}[c]{@{}c@{}}AWS\\ \textit{us-east-1}\end{tabular}} & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}GCP\\ \textit{us-central1}\end{tabular}} \\ \cline{3-12} 
 & & \multicolumn{1}{c|}{\textit{1a}} & \multicolumn{1}{c|}{\textit{1b}} & \multicolumn{1}{c|}{\textit{1c}} & \multicolumn{1}{c|}{\textit{1d}} & \multicolumn{1}{c|}{\textit{1e}} & \multicolumn{1}{c|}{\textit{1f}} & \multicolumn{1}{c|}{\textit{1-a}} & \multicolumn{1}{c|}{\textit{1-b}} & \multicolumn{1}{c|}{\textit{1-c}} & \multicolumn{1}{c|}{\textit{1-f}} \\ \hline
\multicolumn{1}{|c|}{\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}AWS\end{tabular}}} & \textit{1a} & \multicolumn{1}{c|}{15.92±0.59} & \multicolumn{1}{c|}{16.61±0.56} & \multicolumn{1}{r|}{16.43±0.94} & \multicolumn{1}{r|}{17.41±0.92} & \multicolumn{1}{r|}{15.96±0.36} & 16.53±0.43 & \multicolumn{1}{r|}{54.73±27.20} & \multicolumn{1}{r|}{44.47±19.35} & \multicolumn{1}{r|}{61.72±27.19} & 57.10±30.56 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1b} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{16.33±0.80} & \multicolumn{1}{r|}{16.48±0.35} & \multicolumn{1}{r|}{16.29±0.54} & \multicolumn{1}{r|}{16.79±0.80} & 16.39±0.46 & \multicolumn{1}{r|}{77.02±10.93} & \multicolumn{1}{r|}{72.72±13.48} & \multicolumn{1}{r|}{82.52±16.95} & 74.25±14.61 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1d} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{16.68±1.67} & \multicolumn{1}{r|}{16.13±0.74} & \multicolumn{1}{r|}{17.26±1.42} & 16.22±0.63 & \multicolumn{1}{r|}{85.55±32.48} & \multicolumn{1}{r|}{83.43±25.42} & \multicolumn{1}{r|}{90.66±27.30} & 86.51±26.30 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1c} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{r|}{-} & \multicolumn{1}{r|}{17.01±1.74} & \multicolumn{1}{r|}{16.95±0.86} & 17.23±2.04 & \multicolumn{1}{r|}{84.45±19.70} & \multicolumn{1}{r|}{80.26±17.63} & \multicolumn{1}{r|}{76.58±14.73} & 77.55±17.90 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1e} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{r|}{15.8±0.58} & 15.83±0.48 & \multicolumn{1}{r|}{77.42±19.03} & \multicolumn{1}{r|}{72.98±19.13} & \multicolumn{1}{r|}{68.85±19.6} & 71.06±18.81 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1f} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & 15.92±0.19 & \multicolumn{1}{r|}{84.32±20.26} & \multicolumn{1}{r|}{75.87±17.21} & \multicolumn{1}{r|}{77.01±19.37} & 78.73±16.90 \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}GCP\end{tabular}}} & \textit{1-a} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{r|}{6.73±1.29} & \multicolumn{1}{r|}{8.96±1.66} & \multicolumn{1}{r|}{6.26±1.15} & 8.21±1.59 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1-b} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{r|}{10.86±0.38} & \multicolumn{1}{r|}{9.48±1.16} & 10.07±1.49 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1-c} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{r|}{7.15±1.43} & 9.68±1.37 \\ \cline{2-12} 
\multicolumn{1}{|c|}{} & \textit{1-f} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{-} & 10.86±0.43 \\ \hline
\end{tabular}
\end{center}
\end{table*}

Observing the main diagonal in both Tables \ref{tab:rpc_times_training} and \ref{tab:rpc_times_test}, we can see that all AZs in AWS have more homogeneous communication times than the GCP ones. We can also observe that GCP is overall faster than AWS, but the latter is more stable. We can confirm such differences by measuring the average time to exchange a training (or test) message, along with its standard deviation, within a cloud region. The average value and standard deviation of the message exchange in the training message (Table \ref{tab:rpc_times_training}) among all AZs from each region, in the AWS \textit{us-east-1} (resp., GCP \textit{us-central1} ) is 30.73 (resp., 16.32 ) seconds with a standard deviation of 3.09\% (resp., 18.38\%). Moreover, the average time of a training message exchange among the cloud providers (AWS and GCP) is 145.33 seconds, with a standard deviation of 13.60\%. The average values and standard deviation of the exchange time of a test message are analogous. In AWS region \textit{us-east-1} (resp., GPC region \textit{us-central1}) the average value is 16.48 (resp., 8.83) seconds with a standard deviation of 2.97\% (resp., 18.91\%). Finally, the average time for exchanging a test message between providers is 74.82 seconds with a standard deviation of 14.64\%.

Note also that a misplaced task has a great impact on the total FL execution time. For example, if the scheduler allocates the FL server in the main AZ of the east region of AWS (\textit{us-east-1a}) and the clients in the main AZ of the central region of GCP (\textit{us-central1-a}), the communication time is delayed by 3.87 times. 


\subsection{Expected training and evaluation times} \label{subsec:expected_exec_time}
 
Running an application in all available GPU types of a multi-cloud environment to compute the expected training and evaluation times and financial costs is unrealistic. Malta~\etal~\cite{malta2019exploring} proposed a simple equation to calculate the total execution time of a centralized Deep Learning training using only the first two epochs. They observed that all training epochs have similar execution times, except for the first one. We have verified similar behaviour in our previous experiments~\cite{brum2021wcc, brum2021eradrj}. Thus, the Pre-Scheduling module obtains only the times of the first two training and evaluation rounds.

The storage service's access time has also an impact in the total execution time because there are repetitive accesses to the dataset. In turn, the dataset cannot be moved, due to privacy issues. The region, where the VM is deployed, clearly influences the application execution time. In order to observe the impact of accessing the dataset from different regions, the pre-scheduling module obtains the execution times of the first two rounds in a scenario with four clients (with 948 training samples and 522 test samples each) using two different models: the Inception-ResNet v2~\cite{szegedy2017inceptionresnet} and the VGG16~\cite{vgg_paper}. The Inception-ResNet (resp., VGG16) has 164 (resp., 16) layers with more than 54 (resp., 130) million adjustable weights. 

In our experiments, we considered that the datasets were stored in both providers, using the same regions as the previous experiments, the \textit{us-east-1} region of AWS and \textit{us-central1} region of GCP as well as similar VMs to compare the different execution times. We chose the \textit{g4dn.2xlarge} instance of AWS and the \textit{n1-standard-8} instance of GCP. Both of them have eight vCPUs with 32 GB of RAM. The AWS' instance has an NVIDIA T4 GPU with 16 GB of memory and the same GPU model attached to the GCP's instance. 

Tables \ref{tab:times_inception} and \ref{tab:times_vgg16} respectively present the evaluated times for the Inception-ResNet v2 and VGG16 models. Column AWS represents the access time of a \textit{g4dn.2xlarge} deployed in the \textit{us-east-1a} AZ of AWS and column GCP represents the access time of a \textit{n1-standard-8} instance deployed in the \textit{us-central1-a} one. These tables also show the client ID (from 0 to 3), the round of the dummy application, and the step of an FL round (T for training and E for evaluate), each line represents.
%
\begin{table}[h!tbp]
\caption{Times of the Inception-ResNet v2 model (four clients with 5 training epochs per comm. round)} \label{tab:times_inception}
\begin{center}
\footnotesize
\begin{tabular}{|c|c|c|cc|cc|}
\hline
\multirow{2}{*}{Client} & \multirow{2}{*}{Round} & \multirow{2}{*}{Step} & \multicolumn{2}{c|}{DS in AWS} & \multicolumn{2}{c|}{DS in GCP} \\ \cline{4-7} 
 & & & \multicolumn{1}{c|}{AWS} & GCP & \multicolumn{1}{c|}{GCP} & AWS \\ \hline
\multirow{4}{*}{0} & \multirow{2}{*}{1$^{st}$} & T & \multicolumn{1}{c|}{0:15:49} & 0:14:51 & \multicolumn{1}{c|}{0:13:28} & 0:15:16 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:01:04} & 0:01:09 & \multicolumn{1}{c|}{0:00:41} & 0:00:52 \\ \cline{2-7} 
 & \multirow{2}{*}{2$^{nd}$} & T & \multicolumn{1}{c|}{0:05:23} & 0:06:09 & \multicolumn{1}{c|}{0:03:02} & 0:03:37 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:02:57} & 0:03:16 & \multicolumn{1}{c|}{0:00:31} & 0:00:48 \\ \hline
\multirow{4}{*}{1} & \multirow{2}{*}{1$^{st}$} & T & \multicolumn{1}{c|}{0:14:19} & 0:14:37 & \multicolumn{1}{c|}{0:13:39} & 0:13:45 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:01:14} & 0:01:18 & \multicolumn{1}{c|}{0:00:42} & 0:00:51 \\ \cline{2-7} 
 & \multirow{2}{*}{2$^{nd}$} & T & \multicolumn{1}{c|}{0:05:00} & 0:06:05 & \multicolumn{1}{c|}{0:03:06} & 0:03:13 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:02:36} & 0:02:53 & \multicolumn{1}{c|}{0:00:36} & 0:00:46 \\ \hline
\multirow{4}{*}{2} & \multirow{2}{*}{1$^{st}$} & T & \multicolumn{1}{c|}{0:13:52} & 0:15:00 & \multicolumn{1}{c|}{0:13:48} & 0:14:46 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:01:21} & 0:01:23 & \multicolumn{1}{c|}{0:00:41} & 0:00:48 \\ \cline{2-7} 
 & \multirow{2}{*}{2$^{nd}$} & T & \multicolumn{1}{c|}{0:05:48} & 0:06:05 & \multicolumn{1}{c|}{0:03:17} & 0:03:33 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:03:01} & 0:03:03 & \multicolumn{1}{c|}{0:00:31} & 0:00:49 \\ \hline
\multirow{4}{*}{3} & \multirow{2}{*}{1$^{st}$} & T & \multicolumn{1}{c|}{0:13:43} & 0:14:40 & \multicolumn{1}{c|}{0:14:01} & 0:13:58 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:01:05} & 0:01:45 & \multicolumn{1}{c|}{0:00:42} & 0:00:50 \\ \cline{2-7} 
 & \multirow{2}{*}{2$^{nd}$} & T & \multicolumn{1}{c|}{0:05:00} & 0:06:26 & \multicolumn{1}{c|}{0:02:57} & 0:03:16 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:01:42} & 0:04:07 & \multicolumn{1}{c|}{0:00:31} & 0:00:44 \\ \hline
\end{tabular}
\end{center}
\end{table}
%
\begin{table}[h!tbp]
\caption{Times of the VGG16 model (four clients with 5 training epochs per comm. round)} \label{tab:times_vgg16}
\begin{center}
\footnotesize
\begin{tabular}{|c|c|c|cc|cc|}
\hline
\multirow{2}{*}{Client} & \multirow{2}{*}{Round} & \multirow{2}{*}{Step} & \multicolumn{2}{c|}{DS in AWS} & \multicolumn{2}{c|}{DS in GCP} \\ \cline{4-7}
 & & & \multicolumn{1}{c|}{AWS} & GCP & \multicolumn{1}{c|}{GCP} & AWS \\ \hline

\multirow{4}{*}{0} & \multirow{2}{*}{1$^{st}$} & T & \multicolumn{1}{c|}{0:03:58} & 0:03:17 & \multicolumn{1}{c|}{0:02:43} & 0:04:41 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:02:44} & 0:02:31 & \multicolumn{1}{c|}{0:00:38} & 0:00:52 \\ \cline{2-7} 
 & \multirow{2}{*}{2$^{nd}$} & T & \multicolumn{1}{c|}{0:06:52} & 0:07:26 & \multicolumn{1}{c|}{0:02:23} & 0:02:54 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:02:59} & 0:03:38 & \multicolumn{1}{c|}{0:00:31} & 0:00:52 \\ \hline
\multirow{4}{*}{1} & \multirow{2}{*}{1$^{st}$} & T & \multicolumn{1}{c|}{0:03:10} & 0:03:06 & \multicolumn{1}{c|}{0:02:40} & 0:02:46 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:02:26} & 0:02:53 & \multicolumn{1}{c|}{0:00:31} & 0:00:56 \\ \cline{2-7} 
 & \multirow{2}{*}{2$^{nd}$} & T & \multicolumn{1}{c|}{0:07:26} & 0:06:09 & \multicolumn{1}{c|}{0:02:24} & 0:02:55 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:02:08} & 0:03:08 & \multicolumn{1}{c|}{0:00:26} & 0:00:52 \\ \hline
\multirow{4}{*}{2} & \multirow{2}{*}{1$^{st}$} & T & \multicolumn{1}{c|}{0:02:49} & 0:03:30 & \multicolumn{1}{c|}{0:02:49} & 0:04:38 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:02:27} & 0:02:34 & \multicolumn{1}{c|}{0:00:35} & 0:00:52 \\ \cline{2-7} 
 & \multirow{2}{*}{2$^{nd}$} & T & \multicolumn{1}{c|}{0:06:39} & 0:07:27 & \multicolumn{1}{c|}{0:02:23} & 0:03:16 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:02:42} & 0:03:26 & \multicolumn{1}{c|}{0:00:30} & 0:00:46 \\ \hline
\multirow{4}{*}{3} & \multirow{2}{*}{1$^{st}$} & T & \multicolumn{1}{c|}{0:02:56} & 0:03:16 & \multicolumn{1}{c|}{0:02:42} & 0:02:30 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:01:36} & 0:02:41 & \multicolumn{1}{c|}{0:00:36} & 0:01:09 \\ \cline{2-7} 
 & \multirow{2}{*}{2$^{nd}$} & T & \multicolumn{1}{c|}{0:06:24} & 0:07:17 & \multicolumn{1}{c|}{0:02:25} & 0:02:58 \\ \cline{3-7} 
 & & E & \multicolumn{1}{c|}{0:02:49} & 0:02:33 & \multicolumn{1}{c|}{0:00:31} & 0:00:53 \\ \hline
\end{tabular}
\end{center}
\end{table}

We observe a small difference between VMs in AWS and GCP, when comparing the time taken to train and evaluate the datasets in the \textit{us-east-1} region (DS in AWS). Sometimes GCP's VMs finished earlier than the AWS' VMs (\eg, both training times of Client 1 in Table \ref{tab:times_vgg16}). On the other hand, we observed similar execution times when the dataset is in the \textit{us-central1} region (in GCP). This preliminary experiment was conducted with only one instance type per cloud provider and GPU architecture. However, in AWS, there are more than 30 instance types with NVIDIA GPUs~\cite{aws_instances}, and in GCP, there are six different NVIDIA GPU architectures attachable to 27 instance types~\cite{gcp_instances_types}. Therefore, in future experiments, the Pre-Scheduling module should repeat these tests for every instance considered in the framework environment.


\section{Concluding Remarks} \label{sec:conclusion}

This paper proposed a framework to execute Federated Learning applications in a multi-cloud environment minimizing the total execution time and costs. The concept of the whole framework is introduced. The first module, the Pre-Scheduling, is more deeply described and some preliminary experiments were presented and discussed.

As future work, in short-term, we intend to evaluate different scenarios of communication delays and VM failures. Then, we will consider experiments with other FL applications, including known datasets, such as CIFAR-10~\cite{krizhevsky2009cifar10} and MNIST~\cite{deng2012mnist}. Finally, we will focus on the conception of the other modules of the Multi-FedLS framework.

\section*{Acknowledgment}
This research is supported by project CNPq/AWS 440014/2020-4, Brazil, by \textit{Programa Institucional de Internacionaliza\c{c}\~{a}o} (PrInt) from CAPES (process number 88887.310261/2018-00), UNIVERSAL CNPq (process number 145088/2019-7), and the \textit{Coordena\c{c}\~{a}o de Aperfei\c{c}oamento de Pessoal de N\'{i}vel Superior} (CAPES - Finance Code 001).
